Label Encoding for Regression Networks

Deep neural networks are used for a wide range of regression problems. However, there exists a significant gap in accuracy between specialized approaches and generic direct regression in which a network is trained by minimizing the squared or absolute error of output labels. Prior work has shown that solving a regression problem with a set of binary classifiers can improve accuracy by utilizing well-studied binary classification algorithms. We introduce binary-encoded labels (BEL), which generalizes the application of binary classification to regression by providing a framework for considering arbitrary multi-bit values when encoding target values. We identify desirable properties of suitable encoding and decoding functions used for the conversion between real-valued and binary-encoded labels based on theoretical and empirical study. These properties highlight a tradeoff between classification error probability and error-correction capabilities of label encodings. BEL can be combined with off-the-shelf task-specific feature extractors and trained end-to-end. We propose a series of sample encoding, decoding, and training loss functions for BEL and demonstrate they result in lower error than direct regression and specialized approaches while being suitable for a diverse set of regression problems, network architectures, and evaluation metrics. BEL achieves state-of-the-art accuracies for several regression benchmarks. Code is available at https://github.com/ubc-aamodt-group/BEL_regression.

==> sections/all_result_tables.tex <==
\iffalse
\begin{table}[t]
  %\centering
  \setlength\tabcolsep{4pt}
  \caption{Comparison of BEL with different regression approaches. Existing approaches for each benchmark are described in Table~\ref{tab:benchmarks} } 
  \label{tab:compare_regression}
  \scriptsize 
  \begin{tabular}{lL{2.5cm}L{2.5cm}L{2.5cm}L{2.5cm}}
  \toprule
  & \multicolumn{4}{c}{ Error (MAE or NME) / Model size }   \\ \hline
  & \multicolumn{1}{c}{HPE1}        & \multicolumn{1}{c}{HPE2}        & \multicolumn{1}{c}{HPE3}        & \multicolumn{1}{c}{HPE4}         \\ \midrule
  Specialized approach & -           & - &  3.40  / 69.8M & 4.14 / 69.8M  \\ \hline
  Direct regression           & 4.76 {$\pm$0.35} / 23.5M & 5.65 {$\pm$0.13} / 23.5M &   3.40 {$\pm$0.26} / 69.8M &   4.14 {$\pm$0.12} / 69.8M  \\ \hline
  Multiclass classification    &  4.49 {$\pm$0.24} / 24.2M & 5.31 {$\pm$0.05} / 24.8M &  4.54 {$\pm$0.04} / 72.0M &  5.14 {$\pm$0.08} / 72.0M \\ \hline
  BEL        &  \textbf{3.37} {$\pm$0.09} / 23.6M &  \textbf{4.77} {$\pm$0.05} / 23.6M &  \textbf{3.12} {$\pm$0.12} / 69.8M & \textbf{3.90} {$\pm$0.03} / 69.8M  \\ \hline
  BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions & U/GEN-EX/BCE           & U/GEN-EX/BCE           & J/GEN-EX/BCE           & U/GEN-EX/BCE           \\ \bottomrule     
  \end{tabular}
  \begin{tabular}{lL{2.5cm}L{2.5cm}L{2.5cm}L{2.5cm}}
    \toprule
& \multicolumn{1}{c}{FLD1}  & \multicolumn{1}{c}{FLD2} &  \multicolumn{1}{c}{FLD3}    & \multicolumn{1}{c}{FLD4}     \\ \midrule
Specialized approach &  3.45 / { }{ }9.6M  &   \textbf{3.32} / { }{ }9.6M &  \textbf{4.32} / { }{ }9.6M &  1.57 / { }{ }9.6M  \\ \hline
Direct regression           & 3.60 {$\pm$0.02} / 10.2M  & 3.54 {$\pm$0.03} / 10.2M &    4.64 {$\pm$0.03} / 10.2M &  1.51 {$\pm$0.01} / 10.2M  \\ \hline
Multiclass classification    & 3.58 {$\pm$0.03} / 25.4M &  3.51 {$\pm$0.02} / 45.2M &  4.50 {$\pm$0.01} / 61.3M & 1.56 {$\pm$0.01} / 20.1M  \\ \hline
BEL                         &  \textbf{3.34} {$\pm$0.02} / 10.6M &  {3.36} {$\pm$0.02} / 11.2M &   {4.33} {$\pm$0.03} / 11.7M &  \textbf{1.47} {$\pm$0.00} / 10.8M \\ \hline
BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions  & HEXJ/GEN-EX/CE        & J/GEN-EX/CE         & B2JDJ/GEN-EX/CE       & J/GEN-EX/CE       \\ \bottomrule     
\end{tabular}
\begin{tabular}{lL{2.5cm}L{2.5cm}L{2.5cm}L{2.5cm}}
\toprule
&  \multicolumn{1}{c}{AE1}   & \multicolumn{1}{c}{AE2}   & \multicolumn{1}{c}{PN}   &      \\ \midrule
Specialized approach &  2.49 / 21.3M &  3.47 / 21.3M &  4.24 / 1.8M& \\ \hline
Direct regression           & 2.44 {$\pm$0.01} / 23.1M & 3.21 {$\pm$0.02} / 23.1M & 4.24 {$\pm$0.45} / 1.8M& \\ \hline
Multiclass classification    & 2.75 {$\pm$0.03} / 23.1M & 3.38 {$\pm$0.05} / 23.1M & 5.54 {$\pm$0.00} / 1.9M & \\ \hline
BEL                         & \textbf{2.27} {$\pm$0.01} / 23.1M & \textbf{3.11} {$\pm$0.00} / 23.1M &  \textbf{3.11} {$\pm$0.01} / 1.8M& \\ \hline
BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions   &   J/BEL-J/BCE   &  B1JDJ/GEN-EX/L1 & J/GEN/CE    \\ \bottomrule     
\end{tabular}
\end{table}
\fi
\begin{table}[t]
  %\centering
  \setlength\tabcolsep{4pt}
  \caption{Comparison of BEL with different regression approaches. Existing approaches for each benchmark are described in Table~\ref{tab:benchmarks} } 
  \label{tab:compare_regression}
  \scriptsize 
  \begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
  \toprule
  & \multicolumn{4}{c}{ Error (MAE or NME) / Model size }   \\ \hline
  Approach (\% training set used for training)& \multicolumn{1}{c}{HPE1}        & \multicolumn{1}{c}{HPE2}        & \multicolumn{1}{c}{HPE3}        & \multicolumn{1}{c}{HPE4}         \\ \midrule
  BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions &U/GEN-EX/L2 &  U/GEN-EX/BCE&  B1JDJ/BCE/GEN-EX&  U/GEN-EX/BCE \\ \hline
  Specialized approach (80\%) & -           & - &  4.08$\pm$0.11  / 69.8M & 4.69$\pm$0.02 / 69.8M  \\ \hline
  Direct regression (80\%)           & 6.12$\pm$0.02 / 23.5M & 5.97$\pm$0.09 / 23.5M &   4.08$\pm$0.11 / 69.8M &   4.67+4.70 / 69.8M  \\ \hline
  Multiclass classification (80\%)   &  5.38$\pm$0.03 / 24.2M & 5.60$\pm$0.13 / 24.8M & 5.58$\pm$0.04 / 72.0M & 5.86$\pm$0.10 / 72.0M \\ \hline
  BEL (80\%)        &  3.91$\pm$0.08 / 23.6M &  4.91$\pm$0.10 / 23.6M &  3.5$\pm$0.08 / 69.8M & 3.99$\pm$0.04 / 69.8M  \\ \hline
  Specialized approach (100\%)& -           & - &  3.40  / 69.8M & 4.14 / 69.8M  \\ \hline
  Direct regression (100\%)          & 4.76 {$\pm$0.35} / 23.5M & 5.65 {$\pm$0.13} / 23.5M &   3.40 {$\pm$0.26} / 69.8M &   4.14 {$\pm$0.12} / 69.8M  \\ \hline
  Multiclass classification (100\%)   &  4.49 {$\pm$0.24} / 24.2M & 5.31 {$\pm$0.05} / 24.8M &  4.54 {$\pm$0.04} / 72.0M &  5.14 {$\pm$0.08} / 72.0M \\ \hline
  BEL (100\%)       &  3.56$\pm$0.01 / 23.6M &  \textbf{4.77} {$\pm$0.05} / 23.6M &  3.30$\pm$0.04 / 69.8M & \textbf{3.90} {$\pm$0.03} / 69.8M  \\ \bottomrule     
  \end{tabular}
  \begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
    \toprule
  Approach (\% training set used for training) & \multicolumn{1}{c}{FLD1}  & \multicolumn{1}{c}{FLD2} &  \multicolumn{1}{c}{FLD3}    & \multicolumn{1}{c}{FLD4}     \\ \midrule
  BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions  & HEXJ/CE/GEN-EX	& U/CE/GEN-EX	& B1JDJ/CE/GEN-EX	& B1JDJ/CE/GEN-EX \\ \hline
  %Specialized approach &  3.45 / { }{ }9.6M  &   \textbf{3.32} / { }{ }9.6M &  \textbf{4.32} / { }{ }9.6M &  1.57 / { }{ }9.6M  \\ \hline
Direct regression  (80\%)           & 3.70$\pm$0.04 / 10.2M  & 3.69$\pm$0.06 / 10.2M &    4.71$\pm$0.02 / 10.2M &  1.51$\pm$0.01 / 10.2M  \\ \hline
Multiclass classification  (80\%)    & 3.64$\pm$0.02 / 25.4M &  3.68$\pm$0.02 / 45.2M &  4.77$\pm$0.02 / 61.3M & 1.56 {$\pm$0.01} / 20.1M  \\ \hline
BEL                         &  3.35$\pm$0.02 / 10.6M &  3.40$\pm$0.03 / 11.2M &   4.37$\pm$0.01 / 11.7M &  1.48$\pm$0.01 / 10.8M \\ \hline
Specialized approach  (100\%) &  3.45 / { }{ }9.6M  &   \textbf{3.32} / { }{ }9.6M &  \textbf{4.32} / { }{ }9.6M &  1.57 / { }{ }9.6M  \\ \hline
Direct regression (100\%)           & 3.60 {$\pm$0.02} / 10.2M  & 3.54 {$\pm$0.03} / 10.2M &    4.64 {$\pm$0.03} / 10.2M &  1.51 {$\pm$0.01} / 10.2M  \\ \hline
Multiclass classification (100\%)    & 3.58 {$\pm$0.03} / 25.4M &  3.51 {$\pm$0.02} / 45.2M &  4.50 {$\pm$0.01} / 61.3M & 1.56 {$\pm$0.01} / 20.1M  \\ \hline
BEL (100\%)                         &  \textbf{3.34} {$\pm$0.02} / 10.6M &  {3.40} {$\pm$0.02} / 11.2M &   {4.36} {$\pm$0.02} / 11.7M &  \textbf{1.47} {$\pm$0.00} / 10.8M  \\ \bottomrule     
\end{tabular}
\begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
\toprule
Approach (\% training set used for training) &  \multicolumn{1}{c}{AE1}   & \multicolumn{1}{c}{AE2}   & \multicolumn{1}{c}{PN}   &      \\ \midrule
BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions   &   J/BEL-J/BCE   &  B1JDJ/GEN-EX/L1 & J/GEN/CE    \\ \hline
%Specialized approach &  2.49 / 21.3M &  3.47 / 21.3M &  4.24 / 1.8M& \\ \hline
Direct regression  (80\%)          & 2.45 {$\pm$0.01} / 23.1M & 3.34 {$\pm$0.02} / 23.1M & 4.56 {$\pm$0.45} / 1.8M& \\ \hline
Multiclass classification  (80\%)    & 2.85 {$\pm$0.03} / 23.1M & 3.47 {$\pm$0.05} / 23.1M & 6.37 {$\pm$0.00} / 1.9M & \\ \hline
BEL  (80\%)                        & \textbf{2.36} {$\pm$0.01} / 23.1M & \textbf{3.20} {$\pm$0.00} / 23.1M &  \textbf{3.49} {$\pm$0.01} / 1.8M& \\ \hline
Specialized approach (100\%) &  2.49 / 21.3M &  3.47 / 21.3M &  4.24 / 1.8M& \\ \hline
Direct regression (100\%)           & 2.44 {$\pm$0.01} / 23.1M & 3.21 {$\pm$0.02} / 23.1M & 4.24 {$\pm$0.45} / 1.8M& \\ \hline
Multiclass classification (100\%)    & 2.75 {$\pm$0.03} / 23.1M & 3.38 {$\pm$0.05} / 23.1M & 5.54 {$\pm$0.00} / 1.9M & \\ \hline
BEL (100\%)                         & \textbf{2.27} {$\pm$0.01} / 23.1M & \textbf{3.11} {$\pm$0.00} / 23.1M &  \textbf{3.11} {$\pm$0.01} / 1.8M& \\ \bottomrule     
\end{tabular}
\end{table}


\begin{table}[t]
  %\centering
  \setlength\tabcolsep{4pt}
  \caption{Comparison of BEL with different regression approaches. Specialized approaches for each benchmark are described in Table~\ref{tab:benchmarks} } 
  \label{tab:compare_regression}
  \scriptsize 
  \begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
  \toprule
  & \multicolumn{4}{c}{ Error (MAE or NME) / Model size }   \\ \hline
  Approach (\% training set)& \multicolumn{1}{c}{HPE1}        & \multicolumn{1}{c}{HPE2}        & \multicolumn{1}{c}{HPE3}        & \multicolumn{1}{c}{HPE4}         \\ \midrule
  Specialized approach (100\%)& -           & - &  \textbf{3.40}  / 69.8M & 4.14 / 69.8M  \\ \hline
  Specialized approach (80\%) & -           & - &  4.08$\pm$0.11  / 69.8M & 4.69$\pm$0.02 / 69.8M  \\ \hline
  Direct regression (80\%)           & 6.12$\pm$0.02 / 23.5M & 5.97$\pm$0.09 / 23.5M &   4.08$\pm$0.11 / 69.8M &   4.67+4.70 / 69.8M  \\ \hline
  Multiclass classification (80\%)   &  5.38$\pm$0.03 / 24.2M & 5.60$\pm$0.13 / 24.8M & 5.58$\pm$0.04 / 72.0M & 5.86$\pm$0.10 / 72.0M \\ \hline
  BEL (80\%)        &  \textbf{3.91}$\pm$0.08 / 23.6M &  \textbf{4.91}$\pm$0.10 / 23.6M &  \textbf{3.5}$\pm$0.08 / 69.8M & \textbf{3.99}$\pm$0.04 / 69.8M  \\ \hline     
  BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions &U/GEN-EX/L2 &  U/GEN-EX/BCE&  B1JDJ/BCE/GEN-EX&  U/GEN-EX/BCE \\ \bottomrule
  \end{tabular}
  \begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
    \toprule
  Approach (\%training set) & \multicolumn{1}{c}{FLD1}  & \multicolumn{1}{c}{FLD2} &  \multicolumn{1}{c}{FLD3}    & \multicolumn{1}{c}{FLD4}     \\ \midrule
  %Specialized approach &  3.45 / { }{ }9.6M  &   \textbf{3.32} / { }{ }9.6M &  \textbf{4.32} / { }{ }9.6M &  1.57 / { }{ }9.6M  \\ \hline
Specialized approach  (100\%) &  3.45 / { }{ }9.6M  &   \textbf{3.32} / { }{ }9.6M &  \textbf{4.32} / { }{ }9.6M &  1.57 / { }{ }9.6M  \\ \hline
Direct regression  (80\%)           & 3.70$\pm$0.04 / 10.2M  & 3.69$\pm$0.06 / 10.2M &    4.71$\pm$0.02 / 10.2M &  1.51$\pm$0.01 / 10.2M  \\ \hline
Multiclass classification  (80\%)    & 3.64$\pm$0.02 / 25.4M &  3.68$\pm$0.02 / 45.2M &  4.77$\pm$0.02 / 61.3M & 1.56 {$\pm$0.01} / 20.1M  \\ \hline
BEL  (80\%)                         &  \textbf{3.35}$\pm$0.02 / 10.6M &  3.40$\pm$0.03 / 11.2M &   4.37$\pm$0.01 / 11.7M &  \textbf{1.48}$\pm$0.01 / 10.8M \\ \hline  
BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions  & HEXJ/CE/GEN-EX & U/CE/GEN-EX & B1JDJ/CE/GEN-EX & B1JDJ/CE/GEN-EX \\ \bottomrule   
\end{tabular}
\begin{tabular}{L{3.3cm}L{2.35cm}L{2.35cm}L{2.35cm}L{2.35cm}}
\toprule
Approach (\% training set) &  \multicolumn{1}{c}{AE1}   & \multicolumn{1}{c}{AE2}   & \multicolumn{1}{c}{PN}   &      \\ \midrule
%Specialized approach &  2.49 / 21.3M &  3.47 / 21.3M &  4.24 / 1.8M& \\ \hline
Specialized approach (100\%) &  2.49 / 21.3M &  3.47 / 21.3M &  4.24 / 1.8M& \\ \hline
Direct regression  (80\%)          & 2.45 {$\pm$0.01} / 23.1M & 3.34 {$\pm$0.02} / 23.1M & 4.56 {$\pm$0.45} / 1.8M& \\ \hline
Multiclass classification  (80\%)    & 2.85 {$\pm$0.03} / 23.1M & 3.47 {$\pm$0.05} / 23.1M & 6.37 {$\pm$0.00} / 1.9M & \\ \hline
BEL  (80\%)                        & \textbf{2.36} {$\pm$0.01} / 23.1M & \textbf{3.20} {$\pm$0.00} / 23.1M &  \textbf{3.49} {$\pm$0.01} / 1.8M& \\ \hline
BEL $\mathcal{E}/\mathcal{D}/\mathcal{L}$ functions   &   J/BEL-J/BCE   &  B1JDJ/GEN-EX/L1 & J/GEN/CE    \\ \bottomrule
\end{tabular}
\end{table}

==> sections/eval_old.tex <==
\section{Evaluation}
\label{sec:eval}
This section compares different $\{\mathcal{E},\mathcal{D}\}$ functions with direct regression and state-of-the-art approaches\footnote{Bold numbers represent the lowest error overall, and the underlined numbers represent the lowest error achieved by binary-encoded labels.}. We use $\mathcal{D}^{\text{BEL-U}}$~\eqref{eq:8} for BEL-U, $\mathcal{D}^{\text{BEL-J}}$~\eqref{eq:6} for BEL-J, and $\mathcal{D}^{\text{BEL-GEN}}$~\eqref{eq:gen} for rest of the encoding functions.  %Further, we discuss our insights on encoding functions and
Further, we provide an ablation study for different loss and decoding functions. 
%\deval{we can move ablation study to the Appendix for due to space}

\textbf{Head Pose Estimation: }
\begin{table}[t]
  \centering
  \setlength\tabcolsep{2pt}
  \caption{Head poses estimation evaluation for the AFLW2000 (trained on 300W-LP) and BIWI (30\% test split ) datasets.  $200/360$ quantization levels are used for \BEL{ }with ResNet50 and RAFA-Net. } 
  \label{tab:hpe}
  \footnotesize
  \begin{tabular}{L{4.5cm}C{1.5cm}C{1.5cm}cccccccc@{}}
    \toprule
   &   &  &  \multicolumn{4}{c}{Protocol-1} & \multicolumn{4}{c}{Protocol-2}  \\ \midrule
  Architecture &  Feature Extractor &   \#Params (M) &  Yaw & Pitch & Roll & MAE &  Yaw & Pitch & Roll & MAE \\ \hline \hline
  SSR-Net-MD~\cite{ssrnet} { }{ }  (Soft regression) & SSR-Net & 1.1 & 5.14 & 7.09 & 5.89 & 6.01 & 4.24  & 4.35 & 4.19 & 4.26 \\ \hline
  FSA-Caps-Fusion~\cite{fsanet} (Soft regression)  & FSA-Net & 5.1 & 4.50 & 6.08 & 4.64 & 5.07 & 2.89 & 4.29 & 3.60 & 3.60    \\  \hline \hline
  HopeNet ($\alpha$ = 2)~\cite{hopenet} (classification + regression loss) &  ResNet50 &  95.9 & 6.47 & 6.56 & 5.44 & 6.16 & - & - & - & - \\ \hline
  Direct regression (L2 loss) & ResNet50 & 23.1  &  6.34 & 6.90 & 6.87 & 6.71 & 4.62 & 5.24 & 4.43 & 4.76  \\ \hline
  BEL-U ($\theta=10$)  & ResNet50 & 23.1 & 5.22 & \underline{5.71} & 3.95 & 4.96 &  \underline{3.07} & 3.46 & {3.76} & \underline{3.39}\\ \hline 
  BEL-J ($\theta=10$)  & ResNet50 & 23.1 & \underline{4.56} & \underline{5.71} & \underline{3.88} & \underline{4.73} & 3.31 & \underline{3.35} & \underline{3.72} & 3.46  \\ \hline \hline
  RAFA-Net~\cite{rafanet} (Direct Regression)  & RAFA-Net & 69.8 & 3.60 & {{4.92}} & 3.88 & 4.13 & 3.07 & 4.30 & \textbf{{2.82}} & 3.40 \\ \hline 
  BEL-U ($\theta=10$)  & RAFA-Net & 69.8 &\textbf{\underline{3.28}} & \textbf{\underline{4.78}} & 3.55 & \textbf{\underline{3.87}} & 3.07 & 3.90 & {\underline{2.85}} & 3.27\\ \hline 
  BEL-J ($\theta=10$)  & RAFA-Net & 69.8 & 3.37 & 4.83 & \textbf{\underline{3.50}} & 3.90 & \textbf{\underline{3.00}} & \textbf{\underline{3.56}} & {{2.90}} & \textbf{\underline{3.16}}\\ \hline 
  BEL-B1JDJ ($\theta=50$)  & RAFA-Net & 70.1 & 3.75 & 5.14 & 3.97 & 4.29 & 3.18 & 4.12 & 3.36 & 3.55 \\ \hline 
  BEL-B2JDJ ($\theta=50$)  & RAFA-Net & 70.1 & 3.60 & 5.17 & 3.87 & 4.21 & 3.16 & 4.18 & 3.46 & 3.60 \\ \hline 
  BEL-HexJ ($\theta=50$)  & RAFA-Net & 70.1 &4.01 & 5.60 & 3.74 & 4.45 & 3.80 & 5.39 & 3.66 & 4.28 \\ \hline 
  BEL-Hadamard ($\theta=50$)  & RAFA-Net & 70.1 & 5.01 & 5.93 & 5.03 & 5.32 & 4.66 & 6.95 & 5.09 & 5.57 \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \end{table}
Head pose estimation aims to find a human head's pose in terms of three angles: yaw, pitch, and roll. 
In this work, we consider landmark-free 2D head pose estimation. 
We use mean absolute error (MAE) as the evaluation metric.  
We use two evaluation protocols, Protocol-1 (Train dataset: 300W-LP~\cite{300wlp}, Test dataset: AFLW2000~\cite{aflw}) and Protocol-2 (70-30\% train-test split of BIWI dataset~\cite{biwi}). 
We follow the evaluation setting of Hopenet~\cite{hopenet} and FSA-Net~\cite{fsanet}. 
We use RAFA-Net~\cite{rafanet} and ResNet50~\cite{resnet} as feature extractors to evaluate the proposed regression approach and compare with state-of-the-art works that use/propose these architectures as the feature extractor. 

Table~\ref{tab:hpe} compares the test MAE of different approaches for head pose estimation. 
For the RAFA-Net and ResNet50 feature extractors, BEL-U and BEL-J both provide lower MAE compared to the direct regression.
BEL-U and BEL-J results in the lowest MAE  for protocols 1 and 2, and reduces the MAE by up to {$6.5\%$} compared to state-of-the-art landmark-free approaches. 

\textbf{Facial Landmark Detection: }
Facial landmark detection is a problem of detecting the $(x,y)$ coordinates of keypoints in a given face image. 
We use the COFW~\cite{cofw}, AFLW~\cite{aflw}, 300W~\cite{300w}, and WFLW~\cite{lab} datasets for our evaluation. We follow the data augmentation and evaluation protocol used in~\cite{hrnetface}. Normalized mean error (NME) and failure rate (f@8\% and f@10\%) are used as evaluation metrics. 
We use the HRNetV2-W18~\cite{hrnetface} feature extractor pre-trained on ImageNet. 
State-of-the-art approach with HRNetV2-W18~\cite{hrnetface} uses heatmap regression, which minimizes the pixel-level loss between the predicted and target heatmaps. 
The target heatmap is generated by Gaussian distribution around the landmark location. 
For \BEL, we evaluate two strategies. In \BEL-H-x, we convert a heatmap to binary heatmaps using \BEL{ }with $8$ quantization levels. Whereas \BEL-x represents prediction of $(x,y)$ coordinates directly with $256$ quantization levels. 

Table~\ref{tab:fldoverall} compares Test NME for different encodings, direct regression, and state-of-the-art approaches. BEL-H-x achieves poor accuracy as it has a significantly higher number of binary classifiers in the output compared to \BEL{ }for (x,y) coordinates. BEL-B1JDJ outperforms other $\{\mathcal{E},\mathcal{D}\}$ functions, direct regression, and heatmap regression for three out of four datasets. \BEL-x achieves comparable NME for 300W compared to existing works. 
\begin{table}[t]
  \setlength\tabcolsep{4pt}
  \caption{Test NME for Facial landmark detection.  $\theta=10$ is used for 300W/WFLW, and $\theta=30$ is used for COFW/AFLW datasets. }
  \label{tab:fldoverall}
  \footnotesize
  \begin{tabular}{@{}L{4.1cm}cC{1.5cm}C{1cm}C{1cm}C{1cm}C{1cm}}
    \toprule
   &     &  &   \multicolumn{1}{c}{COFW} &    \multicolumn{1}{c}{300W} &    \multicolumn{1}{c}{WFLW} &    \multicolumn{1}{c}{AFLW} \\ \cmidrule{4-7}
  Architecture &  Feature Extractor & \#Params/ GFlops &  Test NME&  Test NME &  Test NME &   Full NME \\  \midrule
  %SAN~\cite{san}               & -           & - & -    & 3.98 & -  & 1.91 \\ \hline
  DAN~\cite{dan}               & -           & - & -    & 3.59 & -  & -    \\ \hline
  DVLN~\cite{dvln}              & VGG16       & - & -    & -    & 6.08  & -    \\ \hline
  LAB (w/o B)~\cite{lab}       & Hourglass   & - & 5.58 & -    & -     & 1.85 \\ \hline
  LAB (w B)~\cite{lab}         & Hourglass   & - & 3.92 & 3.49 & 5.37 & -   \\ \hline \hline
  HRNetV2-W18~\cite{hrnetface} (Heatmaps) & HRNetV2-W18 & 9.6/4.6 & 3.45 &  \textbf{3.32} & 4.60 & 1.57 \\   \hline
  Direct regression (L2 loss) & HRNetV2-W18 & 10.2/4.7  &  3.96 & 3.71 & 5.56 & 1.61  \\ \hline
  Direct regression (L1 loss) & HRNetV2-W18 & 10.2/4.7  &  3.60 & 3.54 & 4.64 & 1.51  \\ \hline
  BEL-H-U             & HRNetV2-W18 & 9.9/4.9  &   4.13   &   -   &  -  &   -   \\ \hline
  BEL-H-J             & HRNetV2-W18 & 9.9/4.9  &   10.17   &   -   &  -  &   -   \\ \hline
  BEL-U             & HRNetV2-W18 & 11.8/4.6  &   3.44   &   {3.47}   &  4.59  &   1.51   \\ \hline
  BEL-J             & HRNetV2-W18 & 11.6/4.6  &  3.43  &  \underline{3.44}    & 4.52   &  1.50    \\ \hline
  BEL-B1JDJ-NRB         & HRNetV2-W18 & 11.5/4.6  &   3.60   &   -  &  -  &   -   \\ \hline
  BEL-B1JDJ         & HRNetV2-W18 & 11.5/4.6  &   \textbf{\underline{3.40}}   &   3.49   &  4.43  &   \textbf{\underline{1.49}}   \\ \hline
  BEL-B2JDJ         & HRNetV2-W18 & 11.6/4.6  &   {3.41}   &   3.45   &  \textbf{\underline{4.41}}  &   1.50   \\ \hline
  BEL-HexJ          & HRNetV2-W18 & 10.6/4.6  &   3.57   &    3.57  &  4.54  &   1.53   \\ \hline
  BEL-Hadamard      & HRNetV2-W18 & 11.8/4.6  &   3.83   &   4.61   & 5.69  &  1.53    \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \end{table}

\textbf{Age Estimation: }
\iffalse
\begin{table}[t]
  \centering
  \setlength\tabcolsep{2pt}
  \caption{Age estimation results comparison for MORPH-II and AFAD datasets.}
  \label{tab:agee}
  \footnotesize
  \begin{tabular}{L{3.1cm}cC{2cm}cc}
    \toprule
   &   &  &  \multicolumn{2}{c}{MAE}  \\ \midrule
  Architecture &  Feature Extractor &   \#Params (M) & MORPH-II & AFAD \\ \hline \hline
  MV Loss~\cite{mvloss} &  &  &  2.41 & - \\ \hline
  CORAL-CNN~\cite{coral} &  & &  2.64 & 3.47 \\ \hline
  Direct regression & ResNet50 & 23.1 & 2.72 & \\ \hline
  BEL-U & ResNet50 & 23.1 & 2.32 & 3.28\\ \hline
  BEL-J & ResNet50 & 23.1 & \textbf{\underline{2.31}} & \textbf{\underline{3.25}} \\ \hline
  BEL-B1JDJ & ResNet50 & 23.1 & 2.32 & 3.27 \\ \hline
  BEL-B2JDJ & ResNet50 & 23.1 & 2.47 & 3.43 \\ \hline
  BEL-HexJ & ResNet50 & 23.1 &  & \\ \hline
  BEL-Hadamard & ResNet50 & 23.1 &   & \\ \hline
  %\cmidrule(r){1-4}decoding
  \end{tabular}
  \end{table}
\fi
\begin{table}[t]
  {
  \centering
  \setlength\tabcolsep{1pt}
  \caption{Age estimation results comparison for MORPH-II and AFAD datasets.}
  \label{tab:agee}
  \footnotesize
  \begin{tabular}{L{2.3cm}ccccccccccc}
      \toprule
  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}OR-\\CNN\cite{agecnn}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MV \\Loss\cite{mvloss}\end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DLDL-\\v2~\cite{dldl}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CORAL-\\CNN~\cite{coralcnn}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Direct\\ regression \end{tabular}} &  \multicolumn{6}{c}{BEL-} \\ \cmidrule(r){7-12}
Approach &  &  &  &  & &  U & J & B1JDJ & B2JDJ & HEXJ & HAD  \\ \midrule
Feature Extractor & - &VGG-16 & ThinAgeNet& ResNet34 &  ResNet50 &  \multicolumn{6}{c}{ResNet50}  \\ \hline 
%\#Params (M) & 1.0& 138.4 & 3.7 & 21.3 & 23.1 & \multicolumn{6}{c}{23.1} \\ \hline
MAE (MORPH-II) & 2.83 & 2.41 & 2.35/1.96* & 2.64 & 2.44 & 2.32 & \textbf{\underline{2.27}} & 2.36 & 2.49 & 2.65 & 2.84 \\ \hline
MAE (AFAD) & 3.51 & -  & -& 3.47 & 3.21 & \textbf{\underline{3.13}} & 3.15 & 3.33 & 3.45 & 3.57 & 3.79 \\ \bottomrule
    %\cmidrule(r){1-4}decoding
    \end{tabular}
  }
    \scriptsize{*uses custom data augmentation for the training}
  \end{table}
We evaluate our approach on MORPH-II~\cite{morphii} an AFAD~\cite{agecnn} datasets. \fisher{add CS5}
In this task, the age of a person is predicted from an image. 
% trained using the same hyperparameters listed above but without pre-training on Imagenet for even comparison with~\cite{}. 
We evaluate our predictions using the MAE of the estimated age and the CS ($\theta = 5$)\deval{@Fisher: what is CS? what is this $\theta$, we should clarify}. We use $64/32$ quantization levels for MORPH-II/AFAD datasets, $\theta=10$ for binary-encoded labels, and ResNet50 (ImageNet pretrained) as our feature extractor. We follow the data augmentation and evaluation protocol used in ~\cite{mvloss}. 

%Overall, our approach BEL-J results in n $24.9\%$ and $1.73\%$ lower error than direct regression and ORBC. 
Table~\ref{tab:agee} compares \BEL{ } with other regression approaches. 
BEL-J achieves $17.7\%$ nd $4.3\%$ improvement over direct regression and domain-specific regression approaches, respectively. 
OR-CNN~\cite{agecnn} and CORAL-CNN~\cite{coralcnn} use ordinal regression by binary classification approach. We achieve significant improvement over these approaches due to the differences in encoding and decoding function, regressor architecture, and training framework. This improvement shows how these different design aspects can be explored to improve regression accuracy by binary classification. \deval{@Fisher, ToDo: add results and other details in the paper}

\textbf{Horizon Line Estimation:}
\begin{table}[]
  \centering
  \setlength\tabcolsep{2pt}
  \caption{Horizon line estimation results on the HLW dataset.}
  \label{tab:hlw}
  \footnotesize
  \begin{tabular}{L{3.1cm}ccccccccc}
  \toprule
  & & & & &  \multicolumn{5}{c}{BEL-} \\ \cmidrule(r){6-10}
  Approach & SLNet~\cite{SLNet}  & SORD~\cite{softcode} & SORD$_{\text{EV}}$~\cite{softcode} & Direct & U & J & B1JDJ & B2JDJ & HEXJ  \\ \midrule
  Feature Extractor & VGG16 &ResNet50 &ResNet50 & ResNet50 & \multicolumn{5}{c}{ResNet50}   \\ \hline 
  \#Params (M) &  - &23.9 & 23.9 & 23.5 & \multicolumn{5}{c}{23.5}  \\ \hline
  AUC (\%) & 82.33 & 88.77 & 89.98 & & & & \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \end{table}
We evaluate our approach on the Horizon Lines in the Wild~\cite{hlw} dataset. In this task, the angle and offset of the horizon line are predicted from an image. We evaluate our predictions using the AUC between the predicted and real angle. We use $256$ quantization levels and $\theta=10$ for binary-encoded labels. We use ResNet50 (ImageNet pretrained) as our feature extractor. We follow the data augmentation and evaluation protocol used in~\cite{softcode}. Table~\ref{tab:hlw} compares \BEL{ } with other regression approaches. BEL-J achieves \red{$1\%$} improvement in the accuracy compared to state-of-the-art regression approaches. \deval{@Fisher: please add details in the table}

We present our observations from the evaluation of different encodings, which can be further used to guide the design space explanation. 
Details on datasets, training parameters, related work for specific tasks, extended results for other evaluation metrics, and discussion of different $\{\mathcal{E},\mathcal{D}\}$ functions are provided in Appendix A3-A6. 
%Overall, BEL-J results in comparable or better accuracy than the existing approaches by making slight modifications in widely used classification networks. 
%, while also achieving greater performance at the same level of sparsity. 
\iffalse
\subsection{Discussion on encoding/decoding functions} \deval{Arrange these points properly}
We believe that one reason behind the increased accuracy of binary-encoded labels is the redundancy added in the output representation, allowing higher tolerance to errors. 
It is essential to design codes so that bit-flip near decision boundaries does not significantly impact the absolute error between target and predicted labels due to the binary classifiers' error probability distribution. 
Thus, it is essential to consider how many bits are different between two codes and their distance from the decision boundaries. 
Also, for some of the datasets, decreasing the number of bits using codes such as B1JDJ and B2JDJ reduces the error, which shows that a high number of output binary classifiers are challenging to optimize for a given training setup. 
Lastly, the size of feature vector needs to be increased for codes with low correlation between the output bits, as we observe that for codes such as B2JDJ and HEXJ, which has low correlation between the binary classifiers, increasing $\theta$ has significant improvement in the accuracy compared to BEL-U and BEL-J codes. 
\begin{table}[b]
  \centering
  \setlength\tabcolsep{5pt}
  \caption{Effect of $\theta$ on the improvement in NME for different encodings over $\theta=5$.}
  \label{tab:bit}
  \footnotesize
  \begin{tabular}{lccc}
    \toprule
  $\theta$/\#parameters in regression layer ($\times 10^6$)& 50/3 & 30/1.8 & 10/0.6  \\ \midrule
  BEL-U & 0.07 & 0.25 & 0.20  \\ \hline
  BEL-J & 0.07 & 0.30& 0.05  \\ \hline
  BEL-B1JDJ & 0.13& 0.11&0.70  \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \end{table}
  \fi
%We can take advantage of the correlation between different bits using lower values of $\theta$ to reduce the number of parameters in the regression layer. Table~\ref{tab:bit} shows the effect of $\theta$ on the MAE for encodings with a different correlation between their output bits. As shown in the figure, MAE for encodings with higher correlation is not much affected by lower values of $\theta$, whereas encodings with less correlation are affected. 
\subsection{Ablation Study}
\label{sec:abl} 
This section further explores different loss and decoding functions, demonstrating the potential of exploring these design aspects together. 

%\textbf{Effect of reflected binary conversion: } We use reflected binary to increase the distance between distant labels. We observe that for facial landmark detection on COFW dataset, reflected binary use improves the NME from $3.60$ to $3.40$ and $4.02$ to $3.41$ for BEL-D1JMJ and BEL-D2JMJ codes. 
\textbf{Impact of loss function}
Table~\ref{tab:loss} compares different combinations of loss functions for facial landmark detection, and head pose estimation. The choice of loss function and decoding function has significant impact on the error, and can be co-designed to improve the accuracy.   
\begin{table}[h]
  \vspace{-5mm}
  \centering
  \setlength\tabcolsep{5pt}
  \caption{Impact of the loss function}
  \label{tab:loss}
  \footnotesize
  \begin{tabular}{lcccccc}
    \toprule
  Task/dataset& $\{\mathcal{E},\mathcal{D}\}$ & BCE & CE & MSE & BCE+MSE & BCE+CE \\ \midrule
  FLD/COFW & BEL-B1JDJ + $\mathcal{D}^{\text{GEN}}$ &3.42 & 3.45 & 9.46 & 3.42 & 3.40 \\ \hline
  FLD/COFW & BEL-J + $\mathcal{D}^{\text{BEL-J}}$ &3.45 & 3.43 & 4.87 & 3.48 & 3.43 \\ \hline
  FLD/COFW & BEL-J + $\mathcal{D}^{\text{GEN-EX}}$ &3.44 & \textbf{3.38} & 4.87 & 3.48 & 3.42 \\ \hline
  HPE/BIWI(ResNet50) & BEL-U + $\mathcal{D}^{\text{BEL-U}}$ & 3.49 & 3.96 & 3.68 & 3.88 & \textbf{3.39} \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \vspace{-5mm}
  \end{table}
\iffalse
\paragraph{Hyperparameter $\theta$:}
We introduce a hyperparameter $\theta$ in the proposed learning approach, where $\theta$ denotes the size of the feature vector before the output layer. Table~\ref{tab:layer} compares test and train MAE for head pose estimation (BIWI dataset protocol 2) for different values of $\theta$. 
%Here $\theta=2048$ indicates direct use of this feature vector.
As shown in the table, the test MAE increases with $\theta$. Whereas, the train MAE slightly decreases with $\theta$, suggesting that the network tends to overfit for higher values of $\theta$, and a smaller feature vector can benefit binary-encoded label regression.  
\begin{table}[]
  \small
  \caption{Effect of feature vector length on MAE}
  \label{tab:layer}
  \begin{center}
    \footnotesize 
  \begin{tabular}{lrrrrr}
  \toprule
$\theta$ & 5 & 10 & 20 & 40 & 2048 \\ \midrule
Test MAE & 3.47 & 3.55 & 3.56 & 3.63 & 3.75  \\ \hline
Train MAE & 0.91 & 0.90 & 0.90 & 0.90 & 0.89  \\ \bottomrule
  \end{tabular}
  \end{center}
  \end{table}
\fi

\textbf{Impact of decoding function: } 
Table~\ref{tab:quanr} compares decoding functions~\eqref{eq:gen} and ~\eqref{eq:genex} that predict quantized and smooth value respectively for different number of quantization intervals. Overall, the GEN-EX decoding function has a lower error than the GEN decoding function due to smoother predictions. This improvement becomes more significant as the number of quantization levels decreases, as GEN-EX reduces the impact of quantization error with fine-grained estimation of decoded value.  The error decreases with quantization step due to lower number of classifiers required, and starts increasing for very high quantization steps ad quantization error becomes very significant. This shows the potential of designing better decoding functions to improve the accuracy further. 
%Table~\ref{tab:quanr} shows the impact of the number of quantization levels on MAE. Quantization error degrades the MAE for a very small number of quantization levels. The improvement achieved by binary-encoded labels is more than quantization error for a higher number of quantization levels, and it outperforms direct regression. 
\begin{table}[h]
  \vspace{-5mm}
  \centering
  \footnotesize 
  \caption{Effect of decoding functions~\eqref{eq:gen} and~\eqref{eq:genex} on MAE}
  \label{tab:quanr}
  %\setlength\tabcolsep{2.2pt} 
  \begin{tabular}{lcccccc}
  \toprule
   & \multicolumn{3}{c}{FLD (COFW)}  & \multicolumn{3}{c}{FLD (300W)} \\ \cline{2-4} \cline{5-7} 
   Quantization step &  4 & 2 & \textbf{1}  &  4 & 2 & \textbf{1}\\ \midrule
  BEL-U + $\mathcal{D}^{\text{GEN}}$ &3.66 & 3.51& 3.46 & 3.79& 3.59& 3.46\\ \hline
  BEL-U + $\mathcal{D}^{\text{GEN-EX}}$ & 3.46 &3.41 & 3.44 & 3.54& 3.47& 3.44\\ \hline
  BEL-J + $\mathcal{D}^{\text{GEN}}$ &  3.65 & 3.49 & 3.44& 3.76 & 3.58 & 3.46 \\ \hline
  BEL-J + $\mathcal{D}^{\text{GEN-EX}}$ & 3.45 &3.40 & 3.43 & 3.52& 3.45 & 3.43 \\ 
\bottomrule
  \end{tabular}%
  \vspace{-5mm}
  \end{table}
  \iffalse
\begin{table}[h]
  \centering
  \footnotesize 
  \caption{Effect of decoding functions~\eqref{eq:gen} and~\eqref{eq:genex} on MAE}
  \label{tab:quanr}
  %\setlength\tabcolsep{2.2pt} 
  \begin{tabular}{lccccccccc}
  \toprule
   & \multicolumn{3}{c}{HPE (Protocol-2)} & \multicolumn{3}{c}{FLD (COFW)}  & \multicolumn{3}{c}{FLD (300W)} \\ \cline{2-4} \cline{5-7} \cline{8-10}
   Quantization step & 4 & 2 & \textbf{1} &  4 & 2 & \textbf{1}  &  4 & 2 & \textbf{1}\\ \midrule
  BEL-U + GEN &  & & &3.66 & 3.51& 3.46 & 3.79& 3.59& 3.46\\ \hline
  BEL-U + GEN-EX &  & & &3.46 &3.41 & 3.44 & 3.54& 3.47& 3.44\\ \hline
  BEL-J + GEN & 4.18 & 3.67 & 3.48 & 3.65 & 3.49 & 3.44& 3.76 & 3.58 & 3.46 \\ \hline
  BEL-J + GEN-EX &  & & &3.45 &3.40 & 3.43 & 3.52& 3.45 & 3.43 \\ 
\bottomrule
  \end{tabular}%
  \end{table}
  \fi

==> sections/methodology.tex <==
\section{Experimental Setup}
We compare proposed encodings with direct regression and state-of-the-art approaches on three challenging regression problems in computer vision. This section gives an overview of the tasks, datasets, network architecture, and evaluation protocols. A detailed description of the datasets, task-specific related work, network architecture, hyperparameters, and the training setup is provided in Appendix~\ref{sec:hpe}-~\ref{sec:pn}. 
%We train direct regression networks using MSE loss. 
We use the PyTorch framework for our implementation. Evaluation metrics for BEL-x and direct regression are averaged over $5$  training runs with random seeds.  \\
\textbf{Head pose estimation: }
Head pose estimation aims to find a human head's pose in terms of three angles: yaw, pitch, and roll. 
In this work, we consider landmark-free 2D head pose estimation, which performs the task based on RGB image information without using facial landmark information. 
%Existing approaches for head pose estimation includes stage-wise soft regression~\cite{ssrnet,fsanet}, coarse-to-fine regression using combination of classification and regression~\cite{deepheadpose,hopenet}, regression via classification~\cite{multilabel}, and ordinal regression~\cite{quatnet}. 
We use mean absolute error (MAE) as the evaluation metric and evaluate the individual yaw, pitch, and roll and overall MAE. 
%We use two evaluation protocols with three widely used datasets: 300W-LP~\cite{300wlp}, BIWI~\cite{biwi}, AFLW2000~\cite{300wlp}. 
We follow the evaluation setting of Hopenet~\cite{hopenet} and FSA-Net~\cite{fsanet}. 
We use two evaluation protocols: in protocol~1, the synthetic 300W-LP dataset is used for training, and the trained network is tested on a real-world AFLW2000 dataset, and in protocol~2, 70\%-30\% splits of BIWI dataset is used for training and testing. 

We use RAFA-Net~\cite{rafanet} and ResNet50~\cite{resnet} as feature extractors to evaluate the proposed regression approach. Further, $360$ quantization levels are used for binary-encoded labels.
We use $\theta=50$ as the feature vector's size for binary-encoded labels. \\
\textbf{Facial landmark detection: }
Facial landmark detection is a problem of detecting the $(x,y)$ coordinates of keypoints in a given face image. 
%The $(x,y)$ coordinates define each keypoint location. 
%Current regression approaches for this tasks includes regression using MSE loss~\cite{SDM}, cascaded regression~\cite{dsrn,7298989}, and coarse to fine regression~\cite{6619290}. State-of-the-art for this task uses heatmap learned by hourglass architecture~\cite{hrnetface,san,dan}.
We use the COFW~\cite{cofw}, AFLW~\cite{aflw}, 300W~\cite{300w}, and WFLW~\cite{lab} datasets for our evaluation. We follow the data augmentation and evaluation protocol used in~\cite{hrnetface}. Normalized mean error (NME) and failure rate (f@8\% and f@10\%) are used as evaluation metrics. We use inter-ocular distance for normalization in the COFW, 300W, and WFLW datasets and the bounding box as a normalization for the AFLW dataset. Further, $256$ quantization levels are used for binary-encoded labels. 
We use the HRNetV2-W18~\cite{hrnetface} feature extractor pre-trained on ImageNet and  $\theta=30$ as the size of the feature vector for binary encoded labels. \\
\textbf{Age estimation: }
We evaluate our approach on MORPH-II\cite{morphii} an AFAD~\cite{agecnn} datasets. 
In this task, the age of a person is predicted from an image. 
% trained using the same hyperparameters listed above but without pre-training on Imagenet for even comparison with~\cite{}. 
We evaluate our predictions using the MAE of the estimated age. We use $100$ quantization levels, and $\theta=10$ for binary-encoded labels. We use \red{ImageNet pretrained ResNet50} as our feature extractor.  
\iffalse
\paragraph{Model compression}
We also evaluate our approach on sparse networks and compare it with direct regression and temperature encoding. 
We perform iterative unstructured pruning and fine-tuning on trained networks~\cite{deepcomp}. 
%Pruning schedule details are provided in the supplementary material. 
% with the sparsity at each stage set to $e$. We prune at the beginning of each stage and train for 20 epochs. The base learning rate is set to $b/2$ and is reduced to $b/10$ after two iterations, and the same mini-batch size is used. 
We use the Erdos-Renyi-Kernel (ERK)~\cite{er,erk} approach to determine sparsity across layers. 
\fi


==> sections/related_work_old.tex <==
\section{Related Work}
\subsection{Regression approaches}
\iffalse
\textbf{Regression methods preserving ordinality:}
Ordinal regression is a regression technique for solving problems where the labels lie on a ranked scale (e.g. 1 to 5 scales, or small/medium/large). A common approach for solving ordinal regression problems is extended binary classification, which decomposes the problem into a set of binary classification problems ~\cite{}.  In comparison to regression via classification (RvC), where a classifier predicts the label for each ordinal class separately, this extended binary classification approach preserves ordinal information across labels and has seen success across a range of tasks ~\cite{}. In these tasks, a continuous regression problem is quantized into an ordinal regression problem. The general formulation for these binary classifiers constructs a single classifier for each boundary between ordinal classes~\cite{}.
% coarse to fine for head pose Wang2019
Ensemble learning has received significant attention in machine learning research ~\cite{?} and has been extended to ordinal regression problems. Improving on the vanilla RvC approach, label diversity ensembles a series of ordinal RvC classifiers using different discrete bin-based representations~\cite{}. Soft targets have also been explored for ordinal regression. Soft regression transformed the ground truth for the RvC approach from a single one-hot target vector to a soft probability distribution of ordinal categories~\cite{}.
(other work has had an applications section as well, presumably to introduce what they evaluate on/cite big labs who tend to review)
\fi
A typical approach for regression problems minimizes mean squared/average error to learn real-valued labels directly. 
%The target label belongs to a continuous range in a regression problem. However, training a neural network for complex regression problems, such as computer vision, often results in poor accuracy and overfitting. 
%The regression problem can be solved by classification. However, this introduces quantization error if the number of classes is too less. If the number of classes is too high, then it suffers from insufficient data samples per class for training. 
The soft regression/deep expectation approach was recently proposed and used for age estimation~\cite{dex,ssrnet}, head pose estimation~\cite{fsanet}, which combines classification and softmax function to find the expected real value of the label. 
Other approaches include coarse-to-fine~\cite{Wang2019}, which combines classification for narrowing the range of the label, and regression for increasing precision of the predicted label.
\subsection{Applications}
\textbf{Head pose estimation:}
Existing approaches for head pose estimation includes stage-wise soft regression~\cite{ssrnet,fsanet}, coarse-to-fine regression using combination of classification and regression~\cite{deepheadpose,hopenet}, regression via classification~\cite{multilabel}, and ordinal regression~\cite{quatnet}. 
SSR-Net~\cite{ssrnet} proposed the use of stage-wise soft regression that uses softmax values of classification output to refine the label. 
FSA-Net ~\cite{fsanet} proposes extending stage-wise estimation to head pose estimation using feature aggregation. 
%Hyperface~\cite{hyperface}, TCDCN~\cite{tcdcn} demonstrates that head pose estimation can be learned jointly with other tasks to improve performance.

\textbf{Facial landmark detection:}
Facial landmark detection is an extensively studied problem used for facial analysis and modeling. 
Common regression approaches for this tasks includes regression using MSE loss~\cite{ssdm,8099876}, cascaded regression~\cite{dsrn,7298989,ccl,fpd}, and coarse to fine regression~\cite{6619290,cfss,cfan}. State-of-the-art methods for this task  learns heatmaps by regression to find facial landmarks. %~\cite{hrnetface,san,dan,lab}. 
SAN~\cite{san} augments training data using temporal information and GAN-generated faces. 
DVLN~\cite{dvln}, CFSS~\cite{cfss}, LAB~\cite{lab}, DSRN~\cite{dsrn} take advantage of correlations between facial landmarks. % to improve performance. 
DAN~\cite{dan} introduces a progressive refinement approach using predicted landmark heatmaps. % passed across stages of a neural network. 
HRNet~\cite{hrnetface} proposes a CNN architecture to maintain high-resolution representations across the network. 
% SAN~\cite{san} augments training data using temporal information and GAN-generated faces, respectively. DVLN~\cite{dvln}, CFSS~\cite{cfss}, LAB~\cite{lab}, DSRN~\cite{dsrn} take advantage of correlations between facial landmarks to improve performance. DAN~\cite{dan} introduces a progressive refinement approach using predicted landmark heatmaps passed across stages of a neural network. HRNet~\cite{hrnetface} proposes a new CNN architecture to maintain high-resolution representations across the network. 
%AnchorFace ~\cite{} demonstrates that anchoring facial landmarks on templates improves regression performance for large poses. CNN-CRF~\cite{} proposed learning facial landmark positions with encoded structural dependencies to preserve geometric relationships.
%
%\textbf{Autonomous driving:}
%End-to-end autonomous driving is a novel task that has become increasingly relevant due to the rise of self-driving vehicles. The autonomous driving model's task is to predict the future driving angle based on a forward-facing image from the perspective of the vehicle. PilotNet~\cite{pilotnet} used a small, application-specific network to succeed within the time constraints of autonomous driving.
%Explaining How a Deep Neural Network Trained with End-to-End Learning Steers a Car
%\textbf{Human pose estimation}
%Human pose estimation is a challenging computer vision problem involving estimation of the positions of key points of a human given an image. Hourglass ~\cite{} constructs a deconvolution head to generate heatmaps for each of the key points. HRNet ~\cite{}, RPN~\cite{} and CPN~\cite{} extended this approach by repeatedly fusing convolutions at multiple scales. Currently, ordinal approaches have been eschewed in favor of deconvolution-based heatmap-prediction approaches.
% Autonomous driving is a novel task that has become increasingly relevant due to the rise of self-driving vehicles. The autonomous driving model's task is to predict the future driving angle based on a forward-facing image from the perspective of the vehicle. Pilotnet~\cite{Explaining How a Deep Neural Network Trained with End-to-End Learning Steers a Car} used a small, application-specific network to succeed within the time constraints of autonomous driving.
% \textbf{Human pose estimation}
% Human pose estimation is a challenging computer vision problem involving estimation of the positions of keypoints of a human given an image. Hourglass ~\cite{} constructs a deconvolution head to generate heatmaps for each of the keypoints. HRNet ~\cite{}, RPN~\cite{} and CPN~\cite{} extended this approach by repeatedly fusing convolutions at multiple scales. Currently, ordinal approaches have been eschewed in favor of deconvolution-based heatmap-prediction approaches.


==> supp_sections/age.tex <==
\newpage
\section{Age Estimation}
\label{sec:a5}
This task aims to predict the age of a person from an image. 
%In this task, the age of a person is predicted from an image. 
We use MORPH-II~\citep{morphii} an AFAD~\citep{agecnn} datasets with data augmentation and evaluation protocols used in ~\citep{mvloss}. 
% trained using the same hyperparameters listed above but without pre-training on Imagenet for even comparison with~\citep{}. 
%We evaluate our predictions using the MAE of the estimated age. 
%e and the CS ($\theta = 5$)\deval{@Fisher: what is CS? what is this $\theta$, we should clarify}. 
%%We use $64$ and $32$ quantization levels for MORPH-II and AFAD datasets and ResNet50 (ImageNet pretrained) as our feature extractor. 
\subsection{Experimental setup}
%Overall, our approach BEL-J results in n $24.9\%$ and $1.73\%$ lower error than direct regression and ORBC. 
We use the MORPH-2~\citep{morphii} and AFAD~\citep{agecnn} datasets for our evaluation. Cumulative Score (CS) and MAE are used as evaluation metrics. We preprocess the MORPH-2 dataset by aligning images first along the average eye position~\citep{mlxtend}, then by re-aligning so that the tip of the nose is in the center of each image. We do not preprocess the AFAD dataset as faces are already centered. Afterwards, face images are resized into $256 \times 256 \times 3$ and randomly cropped to $224 \times 224 \times 3$ for training. For testing, a center crop of $224 \times 224 \times 3$ is taken. 

\paragraph{MORPH-2}
This dataset consists of 55,608 face images with age labels between 16 and 70. The dataset is randomly divided into 39,617 training, 4,398 validation, and 11,001 testing images. 
\paragraph{AFAD}
This dataset consists of 164,432 Asian facial images and age labels between 15 and 40. The dataset is randomly divided into 118,492 training, 13,166 validation, and 32763 testing images. 
\paragraph{Training parameters}
We performed two runs with different random seeds to determine the learning rate between $[0.00001, 0.0001, 0.001]$ and use a batch size of 64 for all experiments. We use ImageNet pretrained weights to initialize the network. 
\begin{table}[h]
    \begin{center}
      \setlength\tabcolsep{6pt}
      \caption{Training parameters for age estimation using MORPH-II and AFAD dataset }
      \label{tab:trage}
      \footnotesize
      \begin{tabular}{L{3cm}C{1cm}ccC{2cm}C{2cm}}
        \toprule
       Optimizer & Epochs & Batch size &  Learning rate & Learning rate schedule  \\  \midrule
      Adam, weight decay=0, momentum=0 & 50 & 64 & 0.0001 & 1/10 at 30, 40 epochs
      \\ \bottomrule
      \end{tabular}
    \end{center}
    \end{table}
\subsection{Related work}
Existing approaches for age estimation include ordinal regression~\citep{agecnn, coralcnn}, soft regression~\citep{ssrnet}, and expected value ordinal regression ~\citep{mvloss, dldl}. OR-CNN~\citep{agecnn} proposed the use of ordinal regression via binary classification to predict the label. CORAL-CNN~\citep{coralcnn} refined this approach by enforcing the ordinality of the model output. SSR-Net~\citep{ssrnet} proposed the use of stage-wise soft regression using the softmax of the classification output to refine the predicted label. MV-Loss~\citep{mvloss} extended the soft regression approach by penalizing the output of the model based on the variance of the age distribution, while DLDL~\citep{dldl} proposed to use the KL-divergence between the softmax output and a generated label distribution to train a model. 
\subsection{Evaluation}
%%%%
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for age estimation for MORPH-II dataset and ResNet50 feature extractor.}
  \label{tab:edlmorph}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 2.32 & \textbf{2.27} & - & - & - & - \\\hline
  GEN-EX & BCE & 2.30 & 2.29 & 2.35 & 2.49 & 2.45 & 2.99 \\\hline
  GEN & BCE & 2.28 & 2.28 & 2.34 & 2.51 & 2.54 & 3.07 \\\hline
  GEN-EX & CE & 2.55 & 2.54 & 2.75 & 2.65 & 2.63 & 12.33 \\\hline
  GEN & CE & 2.60 & 2.58 & 2.61 & 2.66 & 2.61 & 3.10 \\\hline
  GEN-EX & L1 & 2.30 & 2.30 & 2.32 & 2.30 & 2.32 & 2.29 \\
  \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
Table~\ref{tab:edlmorph} compares different combinations of encoding, deocding, and loss functions for BEL approach on MORPH-II dataset and ResNet50 feature extractor. 
\begin{table}[h]
    {
    \centering
    \setlength\tabcolsep{4pt}
    \caption{Age estimation results on MORPH-II dataset. $\theta=10$ is used for BEL.}
    \label{tab:age}
    \footnotesize
    \begin{tabular}{L{4.4cm}cR{2cm}L{2cm}L{2cm}}
    \toprule
    Approach & Feature extractor & \#Parameters (M) & MORPH-II (MAE)& MORPH-II (CS$\theta = 5$)\\ \midrule
    OR-CNN~\citep{agecnn} (Ordinal regression by binary classification ) & - & 1.0 & 2.58 & 0.71 \\ \hline
    MV Loss~\citep{mvloss} (Direct regression) & VGG-16 & 138.4 & 2.41 & 0.889 \\ \hline
    DLDL-v2~\citep{dldl} (Ordinal regression with multi-class classification) & ThinAgeNet & 3.7 & \underline{1.96}* & - \\ \hline
    CORAL-CNN~\citep{coralcnn} (Ordinal regression by binary classification) & ResNet34 & 21.3 & 2.49 & - \\ \hline \hline
    Direct Regression (L2 Loss) & ResNet50 & 23.1 & 2.44 $\pm$ 0.01 & 0.903 $\pm$ 0.002 \\ \hline
    BEL-J/BCE/BEL-J & ResNet50 & 23.1 & \textbf{{2.27}} $\pm$ 0.01& \textbf{\underline{0.928}} $\pm$ 0.001\\   \bottomrule 
    \end{tabular}
    }
    \scriptsize{\\\*Uses custom data augmentation for the training}
    %\vspace{-3mm}
\end{table}
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for age estimation for AFAD dataset and ResNet50 feature extractor.}
  \label{tab:edlafad}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 3.13 & 3.15 & - & - & - & - \\\hline
GEN-EX & BCE & 3.14 & 3.16 & 3.32 & 3.35 & 3.28 & 3.34 \\\hline
GEN & BCE & 3.13 & 3.19 & 3.41 & 3.44 & 3.41 & 3.52 \\\hline
GEN-EX & CE & 3.26 & 3.29 & 3.38 & 3.44 & 3.40 & 3.30 \\\hline
GEN & CE & 3.36 & 3.34 & 3.42 & 3.47 & 3.40 & 3.45 \\\hline
GEN-EX & L1 & 3.13 & 3.12 & \textbf{3.11} & 3.12 & 3.13 & 3.13 \\
  \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
Table~\ref{tab:edlafad} compares different combinations of encoding, deocding, and loss functions for BEL approach on AFAD dataset and ResNet50 feature extractor. 
\begin{table}[h]
  {
  \centering
  \setlength\tabcolsep{4pt}
  \caption{Age estimation results on AFAD dataset. $\theta=10$ is used for BEL.}
  \label{tab:agee}
  \footnotesize
  \begin{tabular}{L{4.4cm}cR{2cm}L{2cm}L{2cm}}
  \toprule
  Approach & Feature extractor & \#Parameters (M) & AFAD (MAE)& AFAD (CS$\theta = 5$)\\ \midrule
  OR-CNN~\citep{agecnn} (Ordinal regression by binary classification ) & - & 1.0 & 3.51 & 0.74 \\ \hline
  CORAL-CNN~\citep{coralcnn} (Ordinal regression by binary classification) & ResNet34 & 21.3 & 3.47 & - \\ \hline \hline
  Direct Regression (L2 Loss) & ResNet50 & 23.1 & 3.21 $\pm$ 0.02 & 0.810 $\pm$ 0.02 \\ \hline
 BEL-B1JDJ/MAE/GEN-EX & ResNet50 & 23.1 & \textbf{\underline{3.11}} $\pm$ 0.01& \textbf{\underline{0.823}} $\pm$ 0.001\\ \bottomrule 
  \end{tabular}
  }
  %\vspace{-3mm}
\end{table}
Table~\ref{tab:age} and Table~\ref{tab:agee} compare \BEL{ }with other regression approaches for MORPH-II and AFAD datasets. 
%BEL-J achieves $17.7\%$ nd $4.3\%$ improvement over direct regression and domain-specific regression approaches, respectively. 
BEL-x provides lower MAE than the direct regression for both datasets, and BEL-B1JDJ/MAE/GEN-EX results in the lowest MAE for the AFAD dataset compared to the state-of-the-art approaches. 
OR-CNN~\citep{agecnn} and CORAL-CNN~\citep{coralcnn} use ordinal regression by binary classification approach. We achieve significant improvement over these approaches due to the differences in encoding and decoding function, regressor architecture, and training framework. This improvement shows the potential of these  design aspects to improve regression accuracy. 

==> supp_sections/auto.tex <==
\newpage
\section{End-to-end Autonomous Driving}
\label{sec:a6}
We evaluate our approach on the NVIDIA PilotNet dataset for end-to-end autonomous driving~\citep{pilotold}. 
In this task, the steering wheel's next angle is predicted from an image of the road. 

\subsection{Experimental setup}
End-to-end autonomous driving is the problem of predicting the target wheel state directly from an image representing the view in front of a car. We use a driving dataset consisting of 45,500 images taken around Rancho Palos Verdes and San Pedro, California~\citep{sully}. We crop images to $256\times 70\times 3$ then resized them to $200\times 66\times 3$. We randomly vary the brightness of the image between $[0.2\times, 1.5\times]$ and randomly perturb the steering direction.
We use PilotNet architecture~\citep{pilotnet} and use $\theta=10$ with $670$ quantization levels for \BEL.  
\paragraph{Training parameters}
We performed two runs with different random seeds to determine the learning rate between $[0.00001, 0.0001, 0.001, 0.01, 0.1]$ and use a batch size of 64 for all experiments. 
\begin{table}[h]
    \begin{center}
      \setlength\tabcolsep{6pt}
      \caption{Training parameters for end-to-end autonomous driving using PilotNet. }
      \label{tab:trage}
      \footnotesize
      \begin{tabular}{L{3cm}C{2cm}ccC{2cm}C{2cm}}
        \toprule
       Optimizer & Epochs & Batch size &  Learning rate & Learning rate schedule  \\  \midrule
       SGD with weight decay=1e-5, momentum=0 & 50 & 64 & 0.1 & 1/10 at 10, 30 epochs
      \\ \bottomrule
      \end{tabular}
    \end{center}
    \end{table}
\subsection{Related work}
End-to-end autonomous driving is a novel task that has become increasingly relevant due to the rise of self-driving vehicles. The autonomous driving model's task is to predict the future driving angle based on a forward-facing image from the perspective of the vehicle. PilotNet~\citep{pilotnet} used a small, application-specific network to succeed within the latency constraints of autonomous driving.
%Explaining How a Deep Neural Network Trained with End-to-End Learning Steers a Car
\subsection{Evaluation}
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for end-to-end autonomous driving for PilotNet dataset and feature extractor.}
  \label{tab:edlpilot}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 4.34 & 3.91 & - & - & - & - \\ \hline
  GEN-EX & BCE & 4.57 & 4.20 & 4.83 & 4.96 & 5.29 & 10.12 \\ \hline
  GEN & BCE & 4.37 & 3.95 & 3.51 & 3.61 & 4.01 & 10.00 \\ \hline
  GEN-EX & CE & 4.30 & 4.16 & 4.99 & 5.87 & 5.39 & 87.17 \\ \hline
  GEN & CE & 3.15 & \textbf{3.11} & 3.14 & 3.21 & 3.64 & 6.20 \\ \hline
  GEN-EX & L1 & 4.10 & 4.11 & 4.34 & 4.34 & 4.11 & 5.09 \\
  \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
Table~\ref{tab:edlpilot} compares different combinations of encoding, deocding, and loss functions for BEL approach on PilotNet dataset and  feature extractor. 
Table~\ref{tab:pilot} compares binary encoded labels with the PilotNet which uses direct regression~\citep{pilotnet}.
\BEL-x results in a significant reduction in the MAE compared to the direct regression approach. 
\begin{table}[h]
    {
    \begin{center}
    \setlength\tabcolsep{4pt}
    \caption{End-to-end autonomous driving results on PilotNet dataset and architecture~\citep{pilotnet,pilotold}.}
    \label{tab:pilot}
    \footnotesize
    \begin{tabular}{L{5.3cm}ccc}
    \toprule
    Approach & Feature extractor & \#Parameters (M) & MAE \\ \midrule
    PilotNet~\citep{pilotnet} & PilotNet & 1.8 & 4.24 $\pm$ 0.45 \\ \hline
    BEL-J/GEN/CE & PilotNet & 1.8 & \textbf{\underline{3.11}} $\pm$ 0.01 \\ 
    \bottomrule 
    \end{tabular}
    \end{center}
    }
\end{table}

==> supp_sections/fdl.tex <==
\section{Facial Landmark Detection}
\label{sec:a4}
Facial landmark detection is a problem of detecting the $(x,y)$ coordinates of keypoints in a given face image. 
%%We u@ext:mathematic.vscode-latexse the COFW~\cite{cofw}, AFLW~\cite{aflw}, 300W~\cite{300w}, and WFLW~\cite{lab} datasets for our evaluation. %We follow the data augmentation and evaluation protocol used in~\cite{hrnetface}. 
Normalized mean error (NME) and failure rate (f@8\% and f@10\%) are used as evaluation metrics. 
%%We use the HRNetV2-W18~\cite{hrnetface} feature extractor. % pre-trained on ImageNet~\cite{imagenet15}. 
The state-of-the-art approach with HRNetV2-W18~\citep{hrnetface} uses heatmap regression, which minimizes the pixel-level loss between the predicted and target heatmaps. 
The target heatmap is generated by Gaussian distribution around the landmark location. 
\BEL-x predicts of $(x,y)$ coordinates directly with $256$ quantization levels. 

\subsection{Experimental setup}
%Current regression approaches for this tasks includes regression using MSE loss~\cite{SDM}, cascaded regression~\cite{dsrn,7298989}, and coarse to fine regression~\cite{6619290}. State-of-the-art for this task uses heatmap learned by hourglass architecture~\cite{hrnetface,san,dan}.
We use the COFW~\citep{cofw}, 300W~\citep{300w}, WFLW~\citep{lab}, and AFLW~\citep{aflw} datasets for the evaluation with data augmentation and evaluation protocol used in~\citep{hrnetface}. Normalized mean error (NME) and failure rate (f@10\%) are used as evaluation metrics. Inter-ocular distance for normalization is used for the COFW, 300W, and WFLW datasets and the bounding box-based normalization is used for the AFLW dataset. Further, $256$ quantization levels are used for binary-encoded labels. 
Data augmentation is performed by random flipping, $0.75-1.25$ scaling, and $\pm 30$ degrees in-plane rotation for all the datasets. 
\\
\paragraph{COFW}
The COFW dataset~\citep{cofw} consists of $1,345$ training and $507$ testing images. Each image is annotated with 29 facial landmarks.  
\paragraph{300W} 
This dataset is a combination of HELEN, LFPW, AFW, XM2VTS, and IBUG datasets. Each image is annotated with 68 facial landmarks. The training dataset consists of $3,148$ images. We evaluate the trained model on four test sets: full test set with $689$ images, common subset with $554$ images from HELEN and LFPW, challenging subset with $135$ images from IBUG, the official test set with $300$ indoor and $300$ outdoor images. 
\paragraph{WFLW}
WFLW dataset consists of $7,500$ training images where each image is annotated with $98$ facial landmarks. Full test dataset consists of $2,500$ images. We use test subsets: large pose ($326$ images), expression ($314$ images), illumination ($698$ images), make-up ($206$ images), occlusion ($736$ images) and blur ($773$ images). 
\paragraph{AFLW} 
Each image has $19$ annotated facial key points in this dataset. 
AFLW dataset consists of $20,000$ training images where each image is annotated with 19 facial landmarks. The full test dataset consists of $4,836$ images, and the frontal test set consists of $1,314$ images.

\paragraph{Training parameters}
Two runs with different random seeds for a learning rate to decide the learning rate. We considered learning rate $\{0.0003,0.0005,0.0007\}$. $\theta \in {10,30}$ is considered for all the codes, and the value is selected for a trade-off between the NME and the model size as a higher value of $\theta$ increases the model size. 
Table~\ref{tab:trfdl} provides a summary of all the training parameters. 
\begin{table}[h]
  \begin{center}
    \setlength\tabcolsep{6pt}
    \caption{Training parameters for facial landmark detection for HRNetV2-W18 feature extractor and direct regression and BEL regression. }
    \label{tab:trfdl}
    \footnotesize
    \begin{tabular}{cC{2.5cm}cC{1cm}C{1.5cm}C{2cm}C{1.5cm}}
      \toprule
    Dataset & Optimizer & Epochs & Batch size &  Learning rate (BEL/Direct regression) & Learning rate schedule  & Training time (GPU hours) \\  \midrule
    COFW & Adam, weight decay=0, momentum = 0 & 60 & 8 & 0.0005/0.0003 & 1/10 after 30 and 50 Epochs &$\frac{1}{2}$ \\ \hline
    300W & Adam, weight decay=0, momentum = 0 & 60 & 8 & 0.0007/0.0003 & 1/10 after 30 and 50 Epochs & 3 \\ \hline
    WFLW & Adam, weight decay=0, momentum = 0 & 60 & 8 & 0.0003/0.0003 & 1/10 after 30 and 50 Epochs & 5 \\ \hline
    AFLW & Adam, weight decay=0, momentum = 0 & 60 & 8 & 0.0005/0.0005 & 1/10 after 30 and 50 Epochs & 8 \\ 
    \bottomrule
    \end{tabular}
  \end{center}
  \end{table}
\paragraph{Network Architecture}
HRNetV2-W18 feature extractor's output is $240$ channels of size $64 \times 64$. For heatmap regression, a $1\times 1$ convolution is used to get $P$ heatmaps of size $64 \times 64$, where $P$ is the number of landmarks. 
\BEL-x predicts of $(x,y)$ coordinates directly with $256$ quantization levels. {Figure}~\ref{fig:hrnet} shows the modified architecture of HRNetV2-W18 for \BEL-x.  
%%In \BEL-H-x, the real-valued heatmaps are converted to binary heatmaps with $8$ quantization levels. Figure~\ref{fig:hrnetc} shows the modified architecture for \BEL-H-x.  
\begin{figure}[h]
\centering
   \includegraphics[width=0.9\textwidth]{figures/hrnet_mod6.pdf}
   \caption{HRNetV2-W18 feature extractor combined with BEL regressor for (x,y) coordinates}
   \label{fig:hrnet}
  \end{figure} 
  \iffalse
\begin{figure}[h]
\centering
   \includegraphics[width=0.9\textwidth]{figures/hrnet_mod6_heatmap.pdf}
   \caption{HRNetV2-W18 feature extractor combined with BEL regressor for heatmaps}
   \label{fig:hrnetc}
\end{figure} 
\fi
\subsection{Related work}
Facial landmark detection is an extensively studied problem used for facial analysis and modeling. 
Common regression approaches for this tasks includes regression using MSE loss~\citep{ssdm,8099876}, cascaded regression~\citep{dsrn,7298989,ccl,fpd}, and coarse to fine regression~\citep{6619290,cfss,cfan}. State-of-the-art methods for this task  learns heatmaps by regression to find facial landmarks. %~\cite{hrnetface,san,dan,lab}. 
SAN~\citep{san} augments training data using temporal information and GAN-generated faces. 
DVLN~\citep{dvln}, CFSS~\citep{cfss}, LAB~\citep{lab}, DSRN~\citep{dsrn} take advantage of correlations between facial landmarks. % to improve performance. 
DAN~\citep{dan} introduces a progressive refinement approach using predicted landmark heatmaps. % passed across stages of a neural network. 
LAB~\citep{lab} also exploits extra boundary information to improve the accuracy. 
LUVLi~\citep{luvli} proposes a landmark's location, uncertainty, and visibility likelihood-based loss. 
~\cite{binaryheatmap} proposes the use of binary heatmaps with pixel-wise binary cross-entropy loss. 
% SAN~\cite{san} augments training data using temporal information and GAN-generated faces, respectively. DVLN~\cite{dvln}, CFSS~\cite{cfss}, LAB~\cite{lab}, DSRN~\cite{dsrn} take advantage of correlations between facial landmarks to improve performance. DAN~\cite{dan} introduces a progressive refinement approach using predicted landmark heatmaps passed across stages of a neural network. HRNet~\cite{hrnetface} proposes a new CNN architecture to maintain high-resolution representations across the network. 
AWing~\citep{awing} proposes adapted wing loss to improve the accuracy of heatmap regression. 
AnchorFace ~\citep{anchorface} demonstrates that anchoring facial landmarks on templates improves regression performance for large poses. 
HRNet~\citep{hrnetface} proposes a CNN architecture to maintain high-resolution representations across the network, and uses heamap regression. 

%%%%%%%%%%%%%%%%%%%%%%Evaluation
\subsection{Evaluation}
%%%COFW
\paragraph{COFW (FDL1)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on NME for facial landmark detection COFW datasets.}
  \label{tab:edlcofw}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 3.47 & 3.45 & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} & \multicolumn{1}{l}{-} \\ \hline
  GEN-EX & BCE & 3.45 & 3.43 & 3.42 & 3.41 & 3.47 & 4.28 \\ \hline
  GEN & BCE & 3.46 & 3.45 & 3.43 & 3.47 & 3.66 & 4.43 \\ \hline
  GEN-EX & CE & 3.37 & 3.37 & 3.38 & 3.41 & \textbf{3.34} & 3.69 \\ \hline
  GEN & CE & 3.44 & 3.44 & 3.44 & 3.49 & 3.57 & 3.69 \\ \hline
  GEN-EX & L1 & 3.44 & 3.41 & 3.45 & 3.47 & 3.41 & 4.52   \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  Table~\ref{tab:edlcofw} compares different combinations of encoding, deocding, and loss functions for BEL approach on COFW dataset. 
Table~\ref{tab:fldcofw} compares different approaches for COFW dataset. BEL-HEXJ/CE/GEN-EX results in the lowest error. 
\begin{table}[h]
\begin{center}
  \setlength\tabcolsep{6pt}
  \caption{Facial landmark detection results on COFW dataset. The failure rate is measured at the threshold 0.1. $\theta=30$ is used for \BEL. }
  \label{tab:fldcofw}
  \footnotesize
  \begin{tabular}{@{}L{4.1cm}cC{1.5cm}ll}
    \toprule
  Approach &  Feature Extractor & \#Params/ GFlops & Test NME & FR$_{0.1}$   \\  \midrule
  LAB (w B)~\citep{lab}         & Hourglass   & 25.1/19.1 & 3.92 & 0.39   \\ \hline 
  AWing~\citep{awing}*         & Hourglass & 25.1/19.1 & 4.94 & -  \\ \hline 
  \hline
  HRNetV2-W18~\citep{hrnetface} (Heatmap regression) & HRNetV2-W18 & 9.6/4.6 & 3.45 &  0.19 \\   \hline
  Direct regression (L2 loss) & HRNetV2-W18 & 10.2/4.7  &  3.96 $\pm$ 0.02 & 0.29  \\ \hline
  Direct regression (L1 loss) & HRNetV2-W18 & 10.2/4.7  &  3.60 $\pm$ 0.02 & 0.29 \\ \hline
  BEL-HEXJ/CE/GEN-EX          & HRNetV2-W18 & 10.6/4.6  &   \textbf{\underline{3.34}} $\pm$ 0.02  & 0.40 \\ \bottomrule
  \end{tabular}
  \scriptsize{\\$*$Uses different data augmentation for the training}
\end{center}
\end{table}

\paragraph{300W (FDL2)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on NME for facial landmark detection 300W datasets.}
  \label{tab:edl300w}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 3.5 & 3.49 & - & - & - & - \\ \hline
  GEN-EX & BCE & 3.48 & 3.46 & 3.43 & 3.42 & 3.38 & 4.71 \\ \hline
  GEN & BCE & 3.50 & 3.49 & 3.45 & 3.45 & 3.55 & 4.78 \\ \hline
  GEN-EX & CE & 3.40 & \textbf{3.36} & 3.37 & 3.41 & 3.37 & 3.62 \\ \hline
  GEN & CE & 3.50 & 3.45 & 3.45 & 3.51 & 3.59 & 3.65 \\ \hline
  GEN-EX & L1 & 3.41 & 3.39 & 3.49 & 3.67 & 3.43 & 4.04 \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  Table~\ref{tab:edl300w} compares different combinations of encoding, deocding, and loss functions for BEL approach on COFW dataset. 
Table~\ref{tab:fld300W} compares different approaches for 300W dataset.approaches.  
\begin{table}[h]
\begin{center}
  \setlength\tabcolsep{3.4pt}
  \caption{Facial landmark detection results on 300W dataset. $\theta=10$ is used for \BEL. }
  \label{tab:fld300W}
  \footnotesize
  \begin{tabular}{@{}L{3.1cm}cC{1.3cm}llll}
    \toprule
  Approach &  Feature Extractor & \#Params/ GFlops & Test & Common & Challenging & Full  \\  \midrule
  DAN~\citep{dan}               & -   & - & -    &  3.19 & 5.24 & 3.59  \\ \hline
  LAB (w B)~\citep{lab}         & Hourglass   & 25.1/19.1 & - & 2.98 & 5.19 & 3.49   \\ \hline 
  AnchorFace~\citep{anchorface} & ShuffleNet-V2   & - & - & 3.12 & 6.19 & 3.72   \\ \hline 
  AWing~\citep{awing}*         & Hourglass & 25.1/19.1 & - & \underline{2.72}& \underline{4.52} & \underline{3.07}  \\ \hline 
  LUVLi~\citep{luvli}   & CU-Net & - &  - & 2.76 & 5.16 & 3.23   \\ \hline
  \hline
  HRNetV2-W18~\citep{hrnetface} (Heatmap regression) & HRNetV2-W18 & 9.6/4.6 &- & 2.87 & \textbf{5.15} & \textbf{3.32}  \\   \hline
  Direct regression (L2 loss) & HRNetV2-W18 & 10.2/4.7  & 4.40 & 3.25 & 5.65 & 3.71 $\pm$ 0.05  \\ \hline
  Direct regression (L1 loss) & HRNetV2-W18 & 10.2/4.7  & 4.26 & 3.10 & 5.42 & 3.54 $\pm$ 0.03 \\ \hline
  BEL-J/CE/GEN-EX             & HRNetV2-W18 & 11.2/4.6  & \textbf{\underline{3.94}} & \textbf{{2.87}} &  5.35  &  {3.36} $\pm$ 0.02   \\ 
  \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \scriptsize{\\$*$Uses different data augmentation for the training}
\end{center}
  \end{table}
\paragraph{WFLW (FDL3)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on NME for facial landmark detection WFLW datasets.}
  \label{tab:edlwflw}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 4.62 & 4.54 & - & - & - & - \\ \hline
  GEN-EX & BCE & 4.6 & 4.51 & 4.43 & 4.38 & 4.37 & 7.18 \\ \hline
  GEN & BCE & 4.62 & 4.53 & 4.44 & 4.42 & 4.55 & 7.14 \\ \hline
  GEN-EX & CE & 4.36 & 4.34 & 4.36 & \textbf{4.33} & 4.34 & 5.15 \\ \hline
  GEN & CE & 4.46 & 4.44 & 4.47 & 4.47 & 4.56 & 4.83 \\ \hline
  GEN-EX & L1 & 4.39 & 4.42 & 4.47 & 4.47 & 4.45 & 4.74\\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  Table~\ref{tab:edlwflw} compares different combinations of encoding, deocding, and loss functions for BEL approach on COFW dataset. 
Table~\ref{tab:fldwflw} compares different approaches for WFLW dataset. 
\begin{table}[h]
  \begin{center}
  \setlength\tabcolsep{2.5pt}
  \caption{Facial landmark detection results (NME) on WFLW test and 6 subsets: pose, expression (expr.), illumination (illu.), make-up (mu.), occlusion (occu.) and blur. $\theta=10$ is used for \BEL.  }
  \label{tab:fldwflw}
  \footnotesize
  \begin{tabular}{@{}L{2.6cm}cC{1.3cm}L{1.6cm}cccccc}
    \toprule
  Approach &  Feature Extractor & \#Params/ GFlops & Test & Pose & Expr. & Illu. & MU & Occu. &Blur  \\  \midrule
  LAB (w B)~\citep{lab} & Hourglass   & 25.1/19.1 & 5.27 & 10.24 & 5.51 & 5.23 & 5.15 & 6.79 & 6.32    \\ \hline 
  AnchorFace~\citep{anchorface}* & HRNetV2-W18   & -/5.3 & \underline{4.32} & 7.51&4.69 &\underline{4.20} &{4.11} &\underline{4.98} & \underline{4.82} \\ \hline 
  AWing~\citep{awing}*         & Hourglass & 25.1/19.1 & 4.36 & \underline{7.38} & \underline{4.58}& 4.32& 4.27& 5.19& 4.96    \\ \hline 
  LUVLi~\citep{luvli}   & CU-Net & - &  4.37  &- &- &-  &-  &-  &- \\ \hline
  \hline
  HRNetV2-W18~\citep{hrnetface} (Heatmap regression) & HRNetV2-W18 & 9.6/4.6 & 4.60 & 7.94 &4.85 &4.55 &4.29 &5.44 & 5.42 \\   \hline
  Direct regression (L2 loss) & HRNetV2-W18 & 10.2/4.7  & 5.56 $\pm$ 0.05 & 10.17 & 6.13 & 5.49 & 5.29 & 6.83  &6.52  \\ \hline
  Direct regression (L1 loss) & HRNetV2-W18 & 10.2/4.7  & 4.64 $\pm$ 0.03  & 8.13& 4.96& 4.49& 4.45& 5.41&5.25\\ \hline
  %0.0501 0.0460 0.0425 0.0738 0.0410 0.0510
  %blue    exp     ill    larg   make    occ
  %\underline{
  BEL-B2JDJ/CE/GEN-EX         & HRNetV2-W18 & 11.7/4.6 &  {\textbf{4.33}} $\pm$ 0.03 &\textbf{\underline{7.38}} &\textbf{4.60} &\textbf{4.25} & \textbf{\underline{4.10}} &\textbf{5.10} &\textbf{5.01}\\ 
   \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \scriptsize{\\$*$Uses different data augmentation for the training}
\end{center}
  \end{table}
\paragraph{AFLW (FDL4)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on NME for facial landmark detection AFLW datasets.}
  \label{tab:edlaflw}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 1.51 & 1.52 & - & - & - & - \\ \hline
  GEN-EX & BCE & 1.50 & 1.50 & \textbf{1.47} & \textbf{1.47} & 1.49 & 1.52 \\ \hline
  GEN & BCE & 1.51 & 1.52 & 1.50 & 1.49 & 1.54 & 1.55 \\ \hline
  GEN-EX & CE & 1.48 & \textbf{1.47} & \textbf{1.47} & \textbf{1.47} & \textbf{1.47} & \textbf{1.47} \\ \hline
  GEN & CE & 1.52 & 1.51 & 1.51 & 1.51 & 1.52 & 1.52 \\ \hline
  GEN-EX & L1 & \textbf{1.47} & \textbf{1.47} & 1.48 & 1.48 & 1.48 & 1.59 \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  Table~\ref{tab:edlaflw} compares different combinations of encoding, deocding, and loss functions for BEL approach on COFW dataset. 
Table~\ref{tab:fldaflw} compares different approaches for AFLW dataset.
\begin{table}[h]
  \begin{center}
  \setlength\tabcolsep{6pt}
  \caption{Facial landmark detection results on AFLW dataset. $\theta=30$ is used for \BEL. }
  \label{tab:fldaflw}
  \footnotesize
  \begin{tabular}{@{}L{4.1cm}cC{1.5cm}ll}
    \toprule
  % &     &  &   \multicolumn{1}{c}{COFW} &    \multicolumn{1}{c}{300W} &    \multicolumn{1}{c}{WFLW} &    \multicolumn{1}{c}{AFLW} \\ \cmidrule{4-7}
  Approach &  Feature Extractor & \#Params/ GFlops & Full & Frontal  \\  \midrule
  LAB (w/o B)~\citep{lab}       & Hourglass   & 25.1/19.1 & 1.85 & 1.62 \\ \hline
  AnchorFace~\citep{anchorface} & ShuffleNet-V2   & - &  1.56 &   \\ \hline 
  LUVLi~\citep{luvli}   & CU-Net & - & \underline{1.39} & \underline{1.19} \\ \hline \hline
  HRNetV2-W18~\citep{hrnetface} (Heatmap regression) & HRNetV2-W18 & 9.6/4.6 & 1.57 & 1.46 \\   \hline 
  Direct regression (L2 loss) & HRNetV2-W18 & 10.2/4.7  &  2.10 $\pm$ 0.02 & 1.71   \\ \hline
  Direct regression (L1 loss) & HRNetV2-W18 & 10.2/4.7  &  1.51 $\pm$ 0.01 & 1.34  \\ \hline
  BEL-J/CE/GEN-EX             & HRNetV2-W18 & 10.8/4.6  & \textbf{1.47} $\pm$ 0.00 & \textbf{1.30}      \\ \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
  \scriptsize{\\$*$Uses different data augmentation for the training}
\end{center}
  \end{table}

%Table~\ref{tab:fldoverall} compares Test NME for different encodings, direct regression, and state-of-the-art approaches. 
%%BEL-H-x achieves poor accuracy due to a significantly higher number of classifiers.  
%%For the HRNetV2-W18 feature extractor, BEL-x provides lower NME than the direct and heatmap regression for COFW and AFLW datasets. 
%%AnchorFace~\cite{anchorface}, which has the lowest NME for the WFLW dataset, uses an Anchor-based approach. This approach is orthogonal to our regression approach and can be combined. 
%BEL-U and BEL-J result in the lowest MAE  for protocols 1 and 2 and reduces the MAE by up to {$6.5\%$} compared to state-of-the-art approaches. 
%%BEL-B1JDJ and BEL-B2JDJ result in the lowest NME for COFW and AFLW datasets compared to the state-of-the-art approaches. 
  \newpage

==> supp_sections/hpe.tex <==
\newpage
\section{Head Pose Estimation}
\label{sec:a3}
Head pose estimation aims to find a human head's pose in terms of three angles: yaw, pitch, and roll. 
In this work, we consider landmark-free 2D head pose estimation. 
We use two evaluation protocols, Protocol-1 (Train dataset: 300W-LP~\citep{300wlp}, Test dataset: AFLW2000~\citep{aflw}) and Protocol-2 (70-30\% train-test split of BIWI dataset~\citep{biwi}) with mean absolute error (MAE) as the evaluation metric. 

Head pose estimation aims to find a human head's pose in terms of three angles: yaw, pitch, and roll. 
This work considers landmark-free 2D head pose estimation, which performs the task based on RGB image information without using facial landmark information. 
\subsection{Experimental setup}
We use two evaluation protocols with three widely used datasets: 300W-LP~\citep{300wlp}, BIWI~\citep{biwi}, AFLW2000~\citep{300wlp} and follow the evaluation setting of Hopenet~\citep{hopenet} and FSA-Net~\citep{fsanet}.
Mean absolute error (MAE) is used as the evaluation metric and the individual yaw, pitch, and roll and overall MAE are evaluated. NVIDIA 2080Ti GPU is used for all the experiments. 
Bold numbers represent the lowest error for the same feature extractor and data augmentation, and the
underlined numbers represent the lowest error overall. Evaluation metrics for BEL and direct regression are
averaged over five training runs with random seeds.
We further explain two protocols in detail. 

Bold numbers represent the lowest error for the same feature extractor and data augmentation, and the
underlined numbers represent the lowest error overall. Evaluation metrics for BEL and direct regression are
averaged over five training runs with random seeds.
\paragraph{Protocol 1:} In this setting, the synthetic 300W-LP dataset is used for training, consisting of $122,450$ samples. The trained network is tested on a real-world AFLW2000 dataset. Yaw, pitch, and roll angles are in the range $[-99,99]$ for both datasets. Table~\ref{tab:trp1} provides a summary of the training parameters. 
\begin{table}[h]
    \begin{center}
      \setlength\tabcolsep{3pt}
      \caption{Training parameters for head pose estimation with protocol 1. }
      \label{tab:trp1}
      \footnotesize
      \begin{tabular}{L{3cm}C{2cm}cC{1cm}C{1.5cm}C{2cm}C{1.5cm}}
        \toprule
      Approach & Optimizer & Epochs & Batch size &  Learning rate & Learning rate schedule  & Training time (GPU hours) \\  \midrule
      ResNet50 with direct regression and BEL & Adam, weight decay=0, momentum = 0 & 20 & 16 & 0.00001 & 1/10 after 10 Epochs & 4 \\ \hline
      RAFA-Net with direct regression~\citep{rafanet} and BEL & RMSProp, momentum=0, rho = 0.9 & 100 & 16 & 0.001 & - & 48 \\ 
      \bottomrule
      \end{tabular}
    \end{center}
    \end{table}
For head pose estimation with ResNet50 architecture (Direct regression and \BEL), two runs with different random seeds for each combination of learning rate $\{0.001,0.0001,0.00001\}$ and batch size $\{8,16\}$ are used for hyperparameter tuning. For data augmentation, images are loosely cropped around the center in the training and testing datasets with random flipping and blurring. Samples with angles in the range [$-99^{\circ}$,$99^{\circ}$] are considered for training and testing. $200$ quantization levels for binary-encoded labels.

For head pose estimation with RAFA-Net, we use the training parameters used in~\citep{rafanet}. 
For data augmentation, we use the approach used in the previous work on RAFA-Net for head pose estimation using direct regression. Angles in the range [$-180^{\circ}$,$180^{\circ}$] with 360 quantization levels are considered for BEL. 

\paragraph{Protocol 2:} BIWI dataset is used for training and evaluation in this protocol. BIWI dataset consists of $24$ videos of $20$ subjects with total $15,128$ frames. Three random splits of 70\%-30\% images are used for training and evaluation. Table~\ref{tab:trp2} provides a summary of the training parameters. 

For head pose estimation with ResNet50 architecture (Direct regression and \BEL), two runs with different random seeds for each combination of learning rate $\{0.001,0.0001,0.00001\}$ and batch size $\{8,16\}$ are used for hyperparameter tuning. For data augmentation, images are loosely cropped around the center in the training and testing datasets with random flipping. 
For the BIWI dataset, the yaw angle is in the range $[-75,75]$, the pitch is in the range $[-65,85]$, and the roll angle is in the range $[-55,45]$. Total $150$ quantization levels are used for yaw and pitch, and $100$ quantization levels are used for roll. 

For head pose estimation with RAFA-Net, we use the training parameters used in~\citep{rafanet}. 
For data augmentation, we use the approach used in the previous work on RAFA-Net for head pose estimation using direct regression. Angles in range [$-180^{\circ}$,$180^{\circ}$] with 360 quantization levels are considered for BEL. 
\begin{table}[h]
  \begin{center}
    \setlength\tabcolsep{3pt}
    \caption{Training parameters for head pose estimation with protocol 1. }
    \label{tab:trp2}
    \footnotesize
    \begin{tabular}{L{3cm}C{2cm}cC{1cm}C{1.5cm}C{2cm}C{1.5cm}}
      \toprule
    Approach & Optimizer & Epochs & Batch size &  Learning rate & Learning rate schedule  & Training time (GPU hours) \\  \midrule
    ResNet50 with direct regression and BEL & Adam, weight decay=0, momentum = 0 & 50 & 8 & 0.0001 & 1/10 after 30 Epochs & 2 \\ \hline
    RAFA-Net with direct regression~\citep{rafanet} and BEL & RMSProp, momentum=0, rho = 0.9 & 100 & 16 & 0.001 & - & 6 \\ 
    \bottomrule
    \end{tabular}
  \end{center}
  \end{table}
\subsection{Related work}
Existing approaches for head pose estimation includes stage-wise soft regression~\citep{ssrnet,fsanet}, combination of classification and regression~\citep{deepheadpose,hopenet}, and ordinal regression~\citep{quatnet}. 
%Head pose estimation has seen significant success from ordinal regression methods, where the model must predict the pose of a human head given an image. This pose is generally represented with 3 degrees of freedom (pitch, yaw, roll). 
SSR-Net~\citep{ssrnet} proposed the use of stage-wise soft regression that uses softmax values of classification output to refine the label. 
FSA-Net ~\citep{fsanet} proposes extending stage-wise estimation to head pose estimation using feature aggregation. 
HopeNet~\citep{hopenet} uses a combination of classification and regression loss to train a model for head pose estimation. 
Whereas QuatNet~\citep{quatnet} solves head pose estimation using a combination of regression L2 loss and ordinal regression loss. 
RAFA-Net~\citep{rafanet} uses an attention based approach for feature extraction with direct regression. 
%Hyperface~\citep{hyperface}, TCDCN~\citep{tcdcn} demonstrates that head pose estimation can be learned jointly with other tasks to improve performance.
\subsection{Evaluation}
\paragraph{Protocol 1 (HPE2 and HPE4)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for head pose estimation with ResNet50 feature extractor.}
  \label{tab:edl1resnet}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 4.78 & 4.84 & - & - & - & - \\ \hline
  GEN-EX & BCE & \textbf{4.77} & 4.84 & 5.43 & 5.09 & 4.94 & 7.84 \\\hline
  GEN & BCE & 4.78 & 4.87 & 5.11 & 5.05 & 5.15 & 8.54 \\\hline
  GEN-EX & CE & 4.93 & 5.04 & 5.04 & 4.97 & 4.79 & 5.64 \\\hline
  GEN & CE & 5.07 & 5.17 & 5.13 & 5.10 & 4.99 & 5.62 \\\hline
  GEN-EX & L1 & 5.05 & 5.18 & 5.19 & 5.09 & 5.17 & 5.07 \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  \begin{table}[]
    \centering
    \footnotesize
    \caption{Comparison of BEL design parameters on MAE for head pose estimation with RAFA-Net feature extractor.}
    \label{tab:edl1rafanet}
    \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
    \toprule
  & \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
    Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
    BEL-J/BEL-U & BCE & 3.94 & 4.00 & - & - & - & - \\\hline
    GEN-EX & BCE & \textbf{3.90} & 3.93 & 10.42 & 15.40 & 29.11 & 9.17 \\\hline
    GEN & BCE & 3.93 & 3.94 & 4.21 & 4.25 & 4.53 & 9.21 \\\hline
    GEN-EX & CE & 4.55 & 4.62 & 4.34 & 4.53 & 4.45 & 5.12 \\\hline
    GEN & CE & 4.68 & 4.75 & 4.46 & 4.61 & 4.63 & 5.29 \\\hline
    GEN-EX & L1 & 4.45 & 5.87 & 5.11 & 9.34 & 10.43 & 17.89 \\\hline
    \bottomrule        
    \end{tabular}
    \end{table}
    %%%%
Table~\ref{tab:edl1resnet} compares different combinations of encoding, deocding, and loss functions for BEL approach on protocol 1 and ResNet50 feature extractor. 
Table~\ref{tab:edl1rafanet} compares different combinations of encoding, deocding, and loss functions for BEL approach on protocol 1 and RAFA-Net feature extractor. 
Table~\ref{tab:hpe1} shows results for protocol 1 with error margin for 95\% confidence interval. For ResNet50 feature extractor, BEL-U/BCE/GEN-EX provides the lowest MAE compared to direct regression and HopeNet~\citep{hopenet}. Whereas, for RAFA-Net feature extractor, BEL-U/BCE/GEN-EX provides the lowest MAE compared to direction regression (L2 loss).   
\begin{table}[h]
  \begin{center}
  \setlength\tabcolsep{6pt}
  \caption{Landmark-free 2D Head poses estimation evaluation for protocol 1.  $200$ and $360$ quantization levels are used for \BEL{ }with ResNet50 and RAFA-Net. } 
  \label{tab:hpe1}
  \footnotesize
  \begin{tabular}{L{3.2cm}C{1.4cm}C{1.1cm}llll@{}}
    \toprule
    Approach & Feature Extractor  & \#Params (M) &  Yaw & Pitch & Roll & MAE  \\ \midrule
  SSR-Net-MD~\citep{ssrnet} { }{ }  (Soft regression) & SSR-Net & 1.1 & 5.14 & 7.09 & 5.89 & 6.01 \\ \hline
  FSA-Caps-Fusion~\citep{fsanet} (Soft regression)  & FSA-Net & 5.1 & 4.50 & 6.08 & 4.64 & 5.07  \\  \hline \hline
  HopeNet* ($\alpha$ = 2)~\citep{hopenet} (classification + regression loss) &  ResNet50 &  23.9 & 6.47 & 6.56 & 5.44 & 6.16 \\ \hline
  Direct regression (L2 loss) & ResNet50 & 23.5  &  6.34 & 6.90 & 6.87  & 6.71 $\pm$ 0.13   \\ \hline
  BEL-U/BCE/GEN-EX  & ResNet50 & 23.6 & \textbf{4.54} & \textbf{5.76} & \textbf{3.96}  & \textbf{4.77} $\pm$ 0.05  \\  \hline \hline
  RAFA-Net~\citep{rafanet} (Direct Regression)  & RAFA-Net & 69.8 & 3.60 & {{4.92}} & 3.88 & 4.13 \\ \hline 
  BEL-U/BCE/GEN-EX  & RAFA-Net & 69.8 &\textbf{\underline{3.28}} & \textbf{\underline{4.78}} & \textbf{\underline{3.55}} & \textbf{\underline{3.90}} $\pm$ 0.03 \\
 \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}\\
  \scriptsize{$*$uses different data preprocessing}
\end{center}
  \end{table}
\paragraph{Protocol 2 (HPE1 and HPE3)}
%%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for head pose estimation with ResNet50 feature extractor.}
  \label{tab:edl2resnet}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 3.38 & 3.65 & - & - & - & - \\\hline
  GEN-EX & BCE & \textbf{3.37} & 3.64 & 5.11 & 8.02 & 4.76 & 7.53 \\\hline
  GEN & BCE & 3.38 & 3.65 & 5.16 & 8.16 & 4.99 & 7.73 \\\hline
  GEN-EX & CE & 4.22 & 3.55 & 3.88 & 4.08 & 4.09 & 5.50 \\\hline
  GEN & CE & 4.25 & 3.62 & 3.93 & 4.06 & 4.39 & 5.48 \\\hline
  GEN-EX & L1 & 3.81 & 3.93 & 3.66 & 3.59 & 5.99 & 4.21 \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
  %%% EDL for COFW
\begin{table}[]
  \centering
  \footnotesize
  \caption{Comparison of BEL design parameters on MAE for head pose estimation with RAFA-Net feature extractor.}
  \label{tab:edl2rafa}
  \begin{tabular}{C{2cm}C{1.5cm}rrrrrr}
  \toprule
& \multicolumn{1}{c}{} & \multicolumn{6}{c}{Encoding function}     \\ \cline{3-8} 
  Decoding function   & Loss function                & \multicolumn{1}{l}{U} & \multicolumn{1}{l}{J} & \multicolumn{1}{l}{B1JDJ} & \multicolumn{1}{l}{B2JDJ} & \multicolumn{1}{l}{HEXJ} & \multicolumn{1}{l}{HAD} \\ \midrule
  BEL-J/BEL-U & BCE & 3.47 & 3.16 & - & - & - & - \\\hline
  GEN-EX & BCE & 3.46 & \textbf{3.12} & 11.67 & 13.29 & 25.42 & 5.75 \\\hline
  GEN & BCE & 3.49 & 3.14 & 3.62 & 3.78 & 4.44 & 5.83 \\\hline
  GEN-EX & CE & 3.82 & 3.91 & 3.52 & 3.49 & 3.98 & 3.98 \\\hline
  GEN & CE & 3.92 & 4.09 & 3.62 & 3.65 & 4.35 & 4.28 \\\hline
  GEN-EX & L1 & 3.72 & 3.60 & 4.31 & 4.29 & 6.61 & 18.69 \\ \bottomrule        
  \end{tabular}
  \end{table}
  %%%%
Table~\ref{tab:edl2resnet} compares different combinations of encoding, deocding, and loss functions for BEL approach on protocol 2 and ResNet50 feature extractor. 
Table~\ref{tab:edl2rafa} compares different combinations of encoding, deocding, and loss functions for BEL approach on protocol 2 and RAFA-Net feature extractor. 
Table~\ref{tab:hpe2} shows results for protocol 2 with error margin for 95\% confidence interval. For ResNet50 feature extractor, BEL-U/BCE/GEN-EX provides the lowest MAE compared to direct regression (L2 loss). Whereas, for RAFA-Net feature extractor, BEL-J/BCE/GEN-EX provides the lowest MAE compared to direction regression (L2 loss). For both the feature extractors, \BEL{ } results in significant decrease in the MAE for pitch compared to direct regression. 
\begin{table}[t]
  \begin{center}
  \setlength\tabcolsep{6pt}
  \caption{Landmark-free 2D Head poses estimation evaluation for protocol 2.  $150$ and $360$ quantization levels are used for \BEL{ }with ResNet50 and RAFA-Net. } 
  \label{tab:hpe2}
  \footnotesize
  \begin{tabular}{L{3.2cm}C{1.4cm}C{1.1cm}llll@{}}
    \toprule
    Approach & Feature Extractor  & \#Params (M) &  Yaw & Pitch & Roll & MAE  \\ \midrule
  SSR-Net-MD~\citep{ssrnet} { }{ }  (Soft regression) & SSR-Net & 1.1  & 4.24  & 4.35 & 4.19 & 4.26 \\ \hline
  FSA-Caps-Fusion~\citep{fsanet} (Soft regression)  & FSA-Net & 5.1 & 2.89 & 4.29 & 3.60 & 3.60    \\  \hline \hline
  Direct regression (L2 loss) & ResNet50 & 23.5  &  4.62  & 5.24  & 4.43 & 4.76 $\pm$ 0.35  \\ \hline
  BEL-U/BCE/GEN-EX  & ResNet50 & 23.6  & \textbf{3.28} & \textbf{\underline{3.36}}  & \textbf{3.44}  & \textbf{3.37} $\pm$ 0.09\\  \hline \hline
  RAFA-Net~\citep{rafanet} (Direct Regression)  & RAFA-Net & 69.8 & 3.07 & 4.30 & 2.82 & 3.40 
 \\ \hline 
  BEL-J/BCE/GEN-EX  & RAFA-Net & 69.8 & \textbf{\underline{2.83}} & \textbf{{3.82}} & \textbf{\underline{2.70}}& \textbf{\underline{3.12}} $\pm$ 0.12\\
  \bottomrule
  %\cmidrule(r){1-4}
  \end{tabular}
\end{center}
\end{table}
\newpage

